MTDNS: Moving Target Defense for Resilient DNS Infrastructure

One of the most critical components of the Internet that an attacker could exploit is the DNS (Domain Name System) protocol and infrastructure. Researchers have been constantly developing methods to detect and defend against the attacks against DNS, specifically DNS flooding attacks. However, most solutions discard packets for defensive approaches, which can cause legitimate packets to be dropped, making them highly dependable on detection strategies. In this paper, we propose MTDNS, a resilient MTD-based approach that employs Moving Target Defense techniques through Software Defined Networking (SDN) switches to redirect traffic to alternate DNS servers that are dynamically created and run under the Network Function Virtualization (NFV) framework. The proposed approach is implemented in a testbed environment by running our DNS servers as separate Virtual Network Functions, NFV Manager, SDN switches, and an SDN Controller. The experimental result shows that the MTDNS approach achieves a much higher success rate in resolving DNS queries and significantly reduces average latency even if there is a DNS flooding attack.

==> Experimental0.tex <==
\section{Experimental}
\label{ex}
\subsection{Setup Overview}
In this section, we introduce tools that we use to implement our Moving Target Defense methodology. These experiments are conducted using standard DNS protocol.

\textbf{Hardware}: We have one Dell Desktop with an i7 CPU with 20 cores, 32GB RAM, and 512GB SSD storage. For the SDN setup, we configure the Desktop as the OVS switch. By redirecting the network connection from OVS to the network stack to the actual Ethernet interface, we can create a structure shown in Figure \ref{fig:Structure}. The experiment is tested under a network throughput of 4.75 Gbps. 



\begin{figure}[h]
\centering
\includegraphics[width=7cm]{fig/p2.png}
\caption{Experiment Topology} 
\vspace{-0.1in}
\label{fig:Structure}
\end{figure}

\textbf{Operating System}: We use Ubuntu server version 20.04.6 LTE as our operating system. We use Ubuntu because installing OVS on Windows is tedious. On the contrary, we just need to use a couple of commands to finish the installation of OVS on Ubuntu. 

\textbf{OVS part}:
We use Open vSwitch version 2.13.8 for the experiment. 

\textbf{SDN controller}:
The controller's job is to continually monitor the DNS flows and write rules to respond to suspicious DNS flows. We want to write our logic directly applicable to the controller instead of fetching statistics from API. RYU uses Python as its programming language, so we can write our logic in Python and directly apply it to the RYU controller. Therefore, we use RYU and write the MTD logic directly to RYU for this project. 

\textbf{DNS Server}:
We use the BIND9 structure to implement our DNS server. We set DNS servers as the recursive resolvers. We propose our methodology using SDN and VNF for the overall structure, so we use virtual machines to implement DNS servers as VNFs. We find that Virtualbox can connect virtual machines to virtual taps created on a virtual bridge, and Virtualbox has a better Graphical User Interface than VM Manager. Virtualbox provides a command line management tool called VBoxManage, which is useful in terms of starting or stopping a VM. Therefore, we use Virtualbox as the virtual machine manager. In terms of DNS servers, since they are VNFs, we install the two DNS servers (i.e., DNS resolvers) on two virtual machines that Virtualbox manages. In order to do this, we create two virtual Ethernet adapters on our host machine, and two virtual DNS servers are connected to the OVS bridge through these two virtual taps on the OVS bridge. One of the DNS servers works as a backup DNS resolver.

\textbf{Comparison between Vbox and Docker}:
We find out that Vbox starts a VM with high latency. This might be because Vbox virtualizes the whole computer hardware infrastructure and allows users to install different OSs on each VM they have created. Yet, Docker virtualizes the kernel OS, which allows OSs that share the same kernel as the host to be virtualized. For example, a user uses Ubuntu as the host OS and may only be able to install OSs from the Linux distribution in the Docker containers. Docker is meant to provide a lightweight solution using kernel virtualization. We are considering using Docker to create containers and connect them to the OVS we have already created. This can be achieved via ovs-docker utility that needs to be downloaded from the OVS GitHub page. The difficulty of using Docker is that we need to use Kubernetes as the orchestrator of the containers we have created. Kubernetes means helmsman or pilot in Greek, and it is used to manage and orchestrate containers. You might think of the role of Kubernetes as the vSphere of VMs. Using Kubernetes with SDN causes extra complexity in the implementation, and we need to use CNI (Container Network Interface) to create an overlay network. This is called OVN (Open Virtual Network). Considering the complexity in implementation, we use VBox's command line management tool to achieve starting VMs on the fly.


\textbf{Host VMs}:
In order to emulate the situation where a legitimate user sends DNS requests to the default DNS server, an attacker attacks the default DNS server. We created two VMs dedicated to this situation. VM Host1 is for the client, and VM Host2 is for the attacker. We use Hping3 on the attacker machine and DNSperf on the client machine.

\textbf{VM Resource Allocation}
We allocated each VM with 2 GB of RAM and 25 GB of storage. Since we use VMs instead of containers, it is resource-consuming to allocate a large storage space and CPU for the VMs. We had run into a situation where VMs were crashed and aborted during the testing phase. Therefore, we allocate even and reasonable resources according to our infrastructure.

\textbf{Backup DNS VM}
The definition for the backup DNS VM is that it helps the default DNS server unload DNS traffic. We have two pre-set thresholds. One is for load-balancing the DNS traffic. Another one is for triggering the startup of the backup DNS server. The second threshold is calculated by taking the half of the load-balancing threshold. We start the backup server first, which can defeat the startup latency introduced by the VM booting process. The flow of the backup DNS VM is that the backup server is started when the VM startup threshold is exceeded. When the load-balancing threshold is exceeded, the DNS traffic between the two servers will be load-balanced by setting an OpenFlow group rule. 

\textbf{Zone File Migration}
We considered using a shared folder to emulate a cloud-like environment for performing zone file transfer. Yet, we found that the master-slave DNS server configuration is less complex in configuration, and this utility comes with the BIND9 server. We use the master-slave DNS configuration or the primary-secondary DNS configuration to migrate the zone file. The idea is that the master server can transfer its zone file to its slave servers. That means that slave servers do not need a zone file configured. The slave servers cannot modify the zone file received from the master server, which is read-only. We found that the zone file transfer is performed using normal traffic, so we set a flow rule to direct the normal traffic, as mentioned. The zone file transfer can be implemented by configuring a DNS server as the master server and the "allow transfer" option in the named.conf.local file. This option allows the admin to specify which IP address or IP range the zone file is going to. The admin may also set the "also-notify" option to notify the slave servers that the zone file is reloaded. This option requires the slave servers to set the "allow-notify" option to accept the notification from the master server properly.

\textbf{SDN and OpenFlow}: 
We utilize SDN capabilities to implement our MTD approaches for the DNS defense. Unlike traditional network structures requiring multiple hardware devices to run and manage the network, SDN centralizes the control plane to a controller. It only leaves the data plane, or the virtual switch, for transmitting data. The SDN is constructed by three elements: an SDN controller, an OpenFlow virtual switch (OVS), and hosts connected to the OVS. The job of the control plane is to manage what and how data is being transmitted while the OVS listens to whatever the controller tells it to do. The controller manages the virtual switch by setting OpenFlow (OF) rules. Network admin can add These rules statically using the OpenFlow vSwitch command line tools or by writing scripts to instruct the controller to add rules according to particular situations. We use the latter for our DNS MTD implementation. OpenFlow rules have two fields that can be utilized to implement the MTD within DNS. They are a field called match and a field called actions. The match field is to match flows that have the defined parameters. In the MTD within DNS case, we match the flows that use UDP protocol, have a port number 53, and are sent from the host virtual machine to one of the DNS servers. As the name suggests, the action field sets actions when a flow is matched with defined parameters. In the DNS MTD case, we set the actions to handle the responses from the backup DNS servers whenever the load balancing is applied. We utilize the Group rule to implement the load balancing between two servers. We use a SELECT Group rule that sets a bucket for each DNS server. We can declare a weight for each bucket. We declare a 50-50 weight for the two buckets in our implementation, which split the DNS traffic into half and load-balance them to two DNS servers. At the development phase, we used a Packet-In to trigger the monitoring task. We found this method introduced an inevitable latency on the first DNS packet after the Packet-In rule is installed. The reason for the latency might be because the controller needs to receive a Packet-In message before installing the DNS request rule. After, we switched to set the DNS request rule as a default rule. This solution eliminates the latency.



\textbf{VM Automation Using Vbox}:
we implement automation using the VBox command line manager called "VBoxManage." It allows us to start and save the state of a VM, which is a good choice for implementing automation. We emulate a middleware environment that controls the start and stop of the VM. The flow of the VM automation is as follows:
\begin{enumerate}
    \item the controller starts the backup DNS server if the VM startup threshold is met.
    \item the controller checks the operational state by using nslookup command to continuously send DNS requests to the backup DNS server until the controller receives a response from the backup DNS server.
    \item The operational state of the backup DNS server is marked as operational
    \item Whenever the load-balancing threshold is met, the backup server is ready to handle the DNS traffic.
\end{enumerate}
Algorithm \ref{alg:VMstartup} is the pseudo-code for the startup part of the VM automation. Algorithm \ref{alg:VMshutdown} is the pseudo-code for the shutdown part of the VM automation.

\begin{algorithm}[h]
\caption{VM Startup Procedure}
\label{alg:VMstartup}
\begin{algorithmic}[1]
    \State Start processing event data
    \For{stat in event}
        \If{stat.PacketCount}
            \State Calculate rate
            \If {\(rate > T1\) \&\& VM is inactive}
                \State Start VM
                \State VM state check
            \If{\(rate > T2\)}
                \State Initiate load balancing procedures
               \EndIf
            \EndIf
        \EndIf
    \EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{VM Shutdown Procedure}
\label{alg:VMshutdown}
\begin{algorithmic}[1]
    \For{group statistic}
        \If{group ID}
            \State Retrieve packet counts for buckets
            \State Calculate rates for each bucket
            \If{rate dropped}
                \State terminate load balancing
                \State switch to default
                \State Shutdown backup VM
            \EndIf
        \EndIf
    \EndFor
\end{algorithmic}
\end{algorithm}


\subsection{Evaluation Metrics}
We are going to use metrics to evaluate the following:
\begin{enumerate}
    \item vDNS Average Latency:
    This metric measures the DNS resolution with and without SDN and Ryu running when a flooding attack is undergoing. In normal use, the two DNS servers we created can have a fair average latency. What if one of them is under attack? Therefore, we are interested in the average latency when a DNS server is under attacked.
    \item vDNS Query Completed Rate:
    This metric is obtained by using DNSperf. This Query Completed Rate reflects not only the performance of DNS servers but also the performance enhancement when SDN and Ryu is in use. In other words, we are interested in the Query Completed Rate when one of the DNS servers is under attacked. Again, we will mimic a flooding attack when obtaining this metric.
    \item Load-Balancing Graph:
    This graph is to visualize the time when the load-balancing is triggered. The data points on the graph are obtained by the calculated packet rate in a two seconds time window. Since we set a 50-50 weight for the two buckets in the group rule respectively, this graph should display a drop, perhaps a half of the spike, in packet rate when the DNS traffic is load-balanced. 
\end{enumerate}



==> Results.tex <==
\section{Results}
\label{result}
\subsection{DNSperf of DNS Server with SDN, Ryu, and Hping3}
Table \ref{table:3} displays the results obtained using load-balancing through SDN and emulating a flooding attack using Hping3. We set a count of 10000 and a payload of 120 bytes for Hping3's DNS requests. We observed that the DNS packets sent by DNSperf have a average packet size of 28 bytes for requests and 70 bytes for responses. Additionally, we use randomly generated IP addresses to perform the flooding attack. For the DNSperf, we use fixed queries per second of 100000 and a duration of 20 seconds. The number of clients is variable to show the differences among the results. We construct the test case by running the DNSperf on the client machine first and then the Hping3 on the attacker machine. We aimed to emulate the situation where the client is doing normal DNS requests, and the attack comes in. We obtained each result by running ten tests with the same parameter and taking the average. All the results reach a query completed rate of around 99.93\% and a latency of around 1.093 ms.
\subsection{DNSperf of DNS Servers with Hping3}
We obtained the results for Table \ref{table:2} using the same parameters and test case mentioned in the DNSperf of DNS Server with SDN, Ryu, and Hping3 section.
\subsection{Comparison}
The query completed rates in Table \ref{table:2} are less than the ones in Table \ref{table:3}, which indicates our proposed method can bring the query completed rate back to around 99.93 percent even though a flooding attack is undergoing. The average latencies in Table \ref{table:2} are higher than in Table \ref{table:3}, indicating that our proposed method can reduce the average latency when a flooding attack occurs by load-balancing the DNS traffic between two servers. 


\subsection{DNS Load-Balancing Results}
Figure \ref{fig:PacketRate} visualizes when the load-balancing between two servers happened. We use flow-based statistics instead of port-based statistics, so we use the default packet rate calculated from the default DNS request rule before the load-balancing job happens and the default DNS server bucket packet rate from the group rule. The zero of the blue line is because the DNSperf we ran on the client machine needs time to load the DNS traffic. The purpose of using DNSperf is to emulate a normal DNS traffic pattern. Before the first spike, the packet rate becomes stable, around 10000 per second. The spike indicates the packet rate exceeds the threshold. If the request rule has a spike shown on the graph, the traffic will be load-balanced between two DNS servers. That is where the group is created, and the group rule is applied to the OVS. The drop after the first spike indicates the start of the load-balancing job. The red line represents the MTD packet rate. It remains zero before the group rule is applied. Once the group rule is installed, we fetch the backup DNS server bucket packet count for the MTD packet rate calculation. When the group rule and the group are deleted, the packet rate becomes zeros again. That is where the zeros are on the red line. Those zeros represent the load-balancing job that is not activated. The two spikes on the graph are mitigated by using MTD. The first load-balancing kicked in at around 28 seconds, and the second load-balancing kicked in at around 82 seconds. We determined the times by finding the intersections between the blue line and the red line.

%\begin{table}[ht]
%\centering
%\begin{tabular}{ |c|c|c|c|c| }
%\hline
%QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
%\hline
%100000 & 125 & 20 & 100\% &1.414\\ 
%\hline
%100000 & 250 & 20 & 100\% &1.226\\
%\hline
%100000 & 500 & 20 & 100\% & 1.377\\ 
%\hline
%\end{tabular}
%\caption{DNSperf of DNS Servers}
%\vspace{-0.2in}
%\label{table:1}
%\end{table}


\begin{table}[ht]
\caption{DNSperf of DNS Servers with Hping3}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
100000 & 125 & 20 & 88.94\% & 3.428 \\ 
\hline
100000 & 250 & 20 & 88.72\% &4.213\\
\hline
100000 & 500 & 20 & 86.41\% &4.133 \\ 
\hline
\end{tabular}
\vspace{-0.2in}
\label{table:2}
\end{table}



\begin{table}[ht]
\caption{DNSperf of DNS Server with SDN, Ryu, and Hping3}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
100000 & 125 & 20 & 99.94\% &1.114 \\ 
\hline
100000 & 250 & 20 & 99.93\% &1.048\\
\hline
100000 & 500 & 20 & 99.93\% & 1.119\\
\hline
\end{tabular}
\vspace{-0.2in}
\label{table:3}
\end{table}
\vspace{0.1in}

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/load-balancing4.png}
\caption{DNS MTD} 
\vspace{-0.1in}
\label{fig:PacketRate}
\end{figure}
\vspace{0.1in}

==> Results0.tex <==
\section{Results}
\label{result}
\subsection{DNSperf of DNS Server with SDN, Ryu, and Hping3}
Table \ref{table:3} displays the results obtained using load-balancing through SDN and emulating a flooding attack using Hping3. We set a count of 10000 and a payload of 120 bytes for Hping3's DNS requests. We observed that the DNS packets sent by DNSperf have a average packet size of 28 bytes for requests and 70 bytes for responses. Additionally, we use randomly generated IP addresses to perform the flooding attack. For the DNSperf, we use fixed queries per second of 100000 and a duration of 20 seconds. The number of clients is variable to show the differences among the results. We construct the test case by running the DNSperf on the client machine first and then the Hping3 on the attacker machine. We aimed to emulate the situation where the client is doing normal DNS requests, and the attack comes in. We obtained each result by running ten tests with the same parameter and taking the average. All the results reach a query completed rate of around 99.93\% and a latency of around 1.093 ms.
\subsection{DNSperf of DNS Servers with Hping3}
We obtained the results for Table \ref{table:2} using the same parameters and test case mentioned in the DNSperf of DNS Server with SDN, Ryu, and Hping3 section.
\subsection{Comparison}
The query completed rates in Table \ref{table:2} are less than the ones in Table \ref{table:3}, which indicates our proposed method can bring the query completed rate back to around 99.93 percent even though a flooding attack is undergoing. The average latencies in Table \ref{table:2} are higher than in Table \ref{table:3}, indicating that our proposed method can reduce the average latency when a flooding attack occurs by load-balancing the DNS traffic between two servers. 


\subsection{DNS Load-Balancing Results}
Figure \ref{fig:PacketRate} visualizes when the load-balancing between two servers happened. We use flow-based statistics instead of port-based statistics, so we use the default packet rate calculated from the default DNS request rule before the load-balancing job happens and the default DNS server bucket packet rate from the group rule. The zero of the blue line is because the DNSperf we ran on the client machine needs time to load the DNS traffic. The purpose of using DNSperf is to emulate a normal DNS traffic pattern. Before the first spike, the packet rate becomes stable, around 10000 per second. The spike indicates the packet rate exceeds the threshold. If the request rule has a spike shown on the graph, the traffic will be load-balanced between two DNS servers. That is where the group is created, and the group rule is applied to the OVS. The drop after the first spike indicates the start of the load-balancing job. The red line represents the MTD packet rate. It remains zero before the group rule is applied. Once the group rule is installed, we fetch the backup DNS server bucket packet count for the MTD packet rate calculation. When the group rule and the group are deleted, the packet rate becomes zeros again. That is where the zeros are on the red line. Those zeros represent the load-balancing job that is not activated. The two spikes on the graph are mitigated by using MTD. The first load-balancing kicked in at around 28 seconds, and the second load-balancing kicked in at around 82 seconds. We determined the times by finding the intersections between the blue line and the red line.

%\begin{table}[ht]
%\centering
%\begin{tabular}{ |c|c|c|c|c| }
%\hline
%QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
%\hline
%100000 & 125 & 20 & 100\% &1.414\\ 
%\hline
%100000 & 250 & 20 & 100\% &1.226\\
%\hline
%100000 & 500 & 20 & 100\% & 1.377\\ 
%\hline
%\end{tabular}
%\caption{DNSperf of DNS Servers}
%\vspace{-0.2in}
%\label{table:1}
%\end{table}


\begin{table}[ht]
\caption{DNSperf of DNS Servers with Hping3}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
100000 & 125 & 20 & 88.94\% & 3.428 \\ 
\hline
100000 & 250 & 20 & 88.72\% &4.213\\
\hline
100000 & 500 & 20 & 86.41\% &4.133 \\ 
\hline
\end{tabular}
\vspace{-0.2in}
\label{table:2}
\end{table}



\begin{table}[ht]
\caption{DNSperf of DNS Server with SDN, Ryu, and Hping3}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
100000 & 125 & 20 & 99.94\% &1.114 \\ 
\hline
100000 & 250 & 20 & 99.93\% &1.048\\
\hline
100000 & 500 & 20 & 99.93\% & 1.119\\
\hline
\end{tabular}
\vspace{-0.2in}
\label{table:3}
\end{table}
\vspace{0.1in}

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/load-balancing4.png}
\caption{DNS MTD} 
\vspace{-0.1in}
\label{fig:PacketRate}
\end{figure}
\vspace{0.1in}











\begin{table}[ht]
\caption{Average Latency and Query Completion Rate of DNS servers with MTDNS}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
5000  & 20 & 99.68\% &0.966 \\ 
\hline
10000  & 20 & 99.79\% &1.006\\
\hline
15000 & 20 & 99.86\% & 1.005\\
\hline
\end{tabular}
%\vspace{-0.2in}
\label{table:3}
\end{table}
\vspace{0.1in}


==> backup/experiments-backup.tex <==
\section{Experimental}
\subsection{Overall Setup}
In this section, we introduce tools that we use to implement our Moving Target Defense methodology. This experiment is conducted using normal DNS protocol.
Hardware:
We have one Dell Desktop with twenty i7 CPUs and five hundred and twenty Gigabyte SSD storage. (more details) For the SDN setup, we configure the Desktop as the OVS switch. By redirecting the network connection from OVS to the IP stack to the actual Ethernet interface, we are able to create a structure that is shown in Figure \ref{fig:Structure}. A detailed explanation of how we set up the environment will be discussed later in the DNS Server part. The experiment is tested under a network bandwidth of 4.74 Gbps. 

\begin{figure}[htp] 
    \centering
    \includegraphics[width=0.3\textwidth]{OVS_structure.png}
    \label{fig:Structure} % optional, for cross-referencing
    \centering
\end{figure}


Operating System:
We use Ubuntu server version 20.04.6 LTE as our operating system. We use Ubuntu because installing OVS on Windows is tedious. On the contrary, we just need to use a couple of commands to finish the installation of OVS on Ubuntu. 

OVS part:
We use Open vSwitch version 2.13.8 for the experiment. 

SDN controller:
The controller's job is to continually monitor the DNS flows and write rules to respond to suspicious DNS flows. We use RYU as the SDN controller. We considered using FloodLight and OpenDayLight as the SDN controller, but we found FloodLight and OpenDayLight are written in JAVA.  We are not familiar with the JAVA language. FloodLight and OpenDayLight can be compatible with Python, but that requires an additional Python program to fetch from the API of either FloodLight or OpenDayLight. In other words, instead of fetching statistics from API, we want to write our logic directly applicable to the controller. RYU uses Python as its programming language, so we can write our logic in Python and directly apply it to the RYU controller. Therefore, we use RYU and write the MTD logic directly to RYU for this project. 

DNS Server:
We use the BIND9 structure to implement our DNS server. We propose our methodology using SDN and VNF for the overall structure, so we use virtual machines to implement DNS servers as VNFs. We use Virtualbox as the virtual machine manager. We make a comparison between VM Manager and Virtualbox. We find that Virtualbox can connect virtual machines to virtual taps created on a virtual bridge, and Virtualbox has a better Graphical User Interface than VM Manager. Therefore, we use Virtualbox as the virtual machine manager. In terms of DNS servers, since they are VNFs, we install the two DNS servers on two virtual machines that Virtualbox manages. What we do is create three virtual Ethernet adapters on our host machine, and the host and two virtual DNS servers are connected to the OVS bridge through these three virtual taps on the OVS bridge. 

Host VMs:
In order to emulate the situation where multiple users are using one of the DNS servers, we create four hosts. Three hosts are normal users, and one host is the attacker machine. On the attacker machine, we use hping3 to generate flooding attacks. On the host VMs, we write a script using the dig command to send DNS requests frequently. (Latency, DNS Perf, expanding nodes)

SDN and OpenFlow: 
We use Software-Defined Networks to implement our DNS MTD. Unlike traditional network structures requiring multiple hardware devices to run and manage the network, Software-Defined Network centralizes the control plane to a controller. It only leaves the data plane, or the virtual switch, for transmitting data. The Software-Defined Network is constructed by three elements: an SDN controller, an OpenFlow virtual switch (OVS), and hosts connected to the OVS. That being said,  the job of the control plane is to manage what and how data is being transmitted, and the virtual switch is a dump switch that listens to whatever the controller tells it to do. The controller manages the virtual switch by setting rules. These rules are called OpenFlow rules. These rules can be added statically by users using the OpenFlow vSwitch command line tools or by users writing scripts to instruct the controller to add rules according to particular situations. We use the latter for our DNS MTD implementation. OpenFlow rules have two fields that can be utilized to implement the DNS MTD. They are a field called match and a field called actions. The match field is to match flows that have the defined parameters. In the DNS MTD case, we match the flows that use UDP protocol, have a port number 53, and are sent from the host virtual machine to one of the DNS servers. As the name suggests, the action field sets actions when a flow is matched with defined parameters. In the DNS MTD case, we set the actions to rotate the IP address of the DNS servers whenever suspicious traffic is detected.

Evaluation:
We are going to use metrics to evaluate the following:
\begin{enumerate}
    \item vDNS resolution latency
    \item latency for Dynamic deployment of vDNS
    \item vDNS resource usage
    \item latency for vDNS zone file migration(if possible)
\end{enumerate}

\subsection{MTD on DNS Flooding Attack}
We implement a simple MTD on DNS flooding attacks. The implementation of MTD on DNS Flooding Attack is straightforward. The MTD process consists of three parts: matching flows, set actions, and triggering IP rotation. The logic is as follows: First, the controller will randomly pick a DNS server IP as the currently active DNS server. Second, the controller sets two rules for monitoring the DNS requests and responses sent from and to the host. Third, the controller sets a rule to direct normal flows. Fourth, the controller periodically fetches the statistics called packet counts from the set DNS response rule that is applied to the OVS. During the experiment, we found that the packet counts from the DNS response rule show a huge difference whenever a flooding attack happens. Thus, we use the packet count in the response rule as the indicator of the occurrence of flooding attacks. Fifth, the controller calculates the transmission rate of the DNS packets. The transmission rate is calculated by dividing the packet difference by the time window of fetching statistics. The packet difference is calculated by subtracting the previous packet counts from the current packet counts. The value of the transmission rate is used as the threshold for detecting the occurrence of flooding attacks. Sixth, whenever the controller finds the transmission rate of the current flow exceeds the threshold, the controller triggers the DNS IP rotation. The controller maintains a list of the DNS server's IP addresses for future rotation, and the rotation only happens within the range of the IP list. After the IP is rotated, the controller updates the DNS traffic flow rules to the rotated DNS server and deletes previous DNS traffic flow rules belonging to the previous DNS server.
The average latency for the DNS server rotation is 10 seconds. We use a timer to record the starting time and the ending time and calculate the latency by subtracting the starting time from the ending time. We construct a list for recording latency and calculate the average latency based on the latency list.
\subsection{MTD on DNS Amplification Attack}
The methodology for detecting DNS amplification attacks is calculating the amplification factor and pairing the response with the corresponding request. The logic behind the pairing scheme is that attackers use spoofed IP addresses and open resolvers to implement the amplification attack. That means the amplified response that targets the victim does not have a corresponding request on the victim's host/resolver.





==> backup/exprimentsbck2.tex <==
\section{Evaluation}
\label{ex}
In this section, we introduce the experimental environment and setup that we use to implement our proposed methodology. These experiments are conducted using traditional DNS protocol in the topology shown in Figure \ref{fig:Structure}. We also provide our experimental metrics and the results.

The source code and scripts developed for the realization of this project have been shared on github at \cite{github}.

\subsection{Setup Overview}
As part of our experimental setup, we define and describe our hardware, Operating System, OVS and SDN, and DNS details.

\textbf{Hardware}: We have Dell Desktops with an i7 CPU with 20 cores, 32GB RAM, and 512GB SSD storage. For the SDN setup, we configure the Desktop as the OVS switch. By redirecting the network connection from OVS to the network stack to the actual Ethernet interface, we can create a structure shown in Figure \ref{fig:Structure}. %The experiment is tested under a network throughput of 4.75 Gbps. 


\begin{figure}[h]
\centering
\includegraphics[width=.65\linewidth]{fig/p2.png}
\caption{Experiment Topology} 
\vspace{-0.1in}
\label{fig:Structure}
\end{figure}

\textbf{Operating System}: We use Ubuntu server version 20.04.6 LTE as our operating system. We use Ubuntu because installing OVS on Windows is tedious. On the contrary, we just need to use a couple of commands to finish the installation of OVS on Ubuntu. 

\textbf{OVS and SDN controller}:
We use Open vSwitch version 2.13.8 for the experiment. 
We use RYU as the SDN Controller and write the MTD logic directly to RYU. The controller's job is to continually monitor the DNS flows and write rules to respond to and provide resiliency against suspicious or just increasing DNS requests. We write our logic directly applicable to the controller instead of fetching statistics from API. 

\textbf{DNS Server}:
We use the BIND9~\cite{jinmei2006implementation} structure to implement our DNS server. We set DNS servers as the recursive resolvers. We propose our methodology using SDN and VNF for the overall structure, so we use virtual machines (VM) to implement DNS servers as VNFs. We find that Virtualbox can connect VMs to virtual taps created on a virtual bridge, and Virtualbox has a better Graphical User Interface than VM Manager. Virtualbox provides a command line management tool called VBoxManage, which is useful in terms of starting or stopping a VM. Therefore, we use Virtualbox as the VM manager. In terms of DNS servers, since they are VNFs, we install the two DNS servers (i.e., DNS resolvers) on two VMs that Virtualbox manages. In order to do this, we create two virtual Ethernet adapters on our host machine, and two virtual DNS servers are connected to the OVS bridge through these two virtual taps on the OVS bridge. One of the DNS servers works as a backup DNS resolver.

\textbf{Vbox}:
We find out that Vbox starts a VM with high latency. This might be because Vbox virtualizes the whole computer hardware infrastructure and allows users to install different OSs on each VM they have created. Yet, Docker virtualizes the kernel OS, which allows OSs that share the same kernel as the host to be virtualized. For example, a user uses Ubuntu as the host OS and may only be able to install OSs from the Linux distribution in the Docker containers. Docker is meant to provide a lightweight solution using kernel virtualization. We are considering using Docker to create containers and connect them to the OVS we have already created. This can be achieved via ovs-docker utility that needs to be downloaded from the OVS GitHub page. The difficulty of using Docker is that we need to use Kubernetes as the orchestrator of the containers we have created. Kubernetes means helmsman or pilot in Greek, and it is used to manage and orchestrate containers. You might think of the role of Kubernetes as the vSphere of VMs. Using Kubernetes with SDN causes extra complexity in the implementation, and we need to use CNI (Container Network Interface) to create an overlay network. This is called OVN (Open Virtual Network). Considering the complexity in implementation, we use VBox's command line management tool to achieve starting VMs on the fly.


\textbf{Host VMs}:
In order to emulate the situation where a legitimate user sends DNS requests to the default DNS server, an attacker attacks the default DNS server. We created two VMs dedicated to this situation. VM Host1 is for the client, and VM Host2 is for the attacker. We use Hping3 on the attacker machine and DNSperf on the client machine.

\textbf{VM Resource Allocation}
We allocated each VM with 2 GB of RAM and 25 GB of storage. Since we use VMs instead of containers, it is resource-consuming to allocate a large storage space and CPU for the VMs. We had run into a situation where VMs were crashed and aborted during the testing phase. Therefore, we allocate even and reasonable resources according to our infrastructure.

\textbf{Backup DNS VM}
The definition for the backup DNS VM is that it helps the default DNS server unload DNS traffic. We have two pre-set thresholds. One is for load-balancing the DNS traffic. Another one is for triggering the startup of the backup DNS server. The second threshold is calculated by taking the half of the load-balancing threshold. We start the backup server first, which can defeat the startup latency introduced by the VM booting process. The flow of the backup DNS VM is that the backup server is started when the VM startup threshold is exceeded. When the load-balancing threshold is exceeded, the DNS traffic between the two servers will be load-balanced by setting an OpenFlow group rule. 

\textbf{Zone File Migration}
We considered using a shared folder to emulate a cloud-like environment for performing zone file transfer. Yet, we found that the master-slave DNS server configuration is less complex in configuration, and this utility comes with the BIND9 server. We use the master-slave DNS configuration or the primary-secondary DNS configuration to migrate the zone file. The idea is that the master server can transfer its zone file to its slave servers. That means that slave servers do not need a zone file configured. The slave servers cannot modify the zone file received from the master server, which is read-only. We found that the zone file transfer is performed using normal traffic, so we set a flow rule to direct the normal traffic, as mentioned. The zone file transfer can be implemented by configuring a DNS server as the master server and the "allow transfer" option in the named.conf.local file. This option allows the admin to specify which IP address or IP range the zone file is going to. The admin may also set the "also-notify" option to notify the slave servers that the zone file is reloaded. This option requires the slave servers to set the "allow-notify" option to accept the notification from the master server properly.

\textbf{SDN and OpenFlow}: 
We utilize SDN capabilities to implement our MTD approaches for the DNS defense. Unlike traditional network structures requiring multiple hardware devices to run and manage the network, SDN centralizes the control plane to a controller. It only leaves the data plane, or the virtual switch, for transmitting data. The SDN is constructed by three elements: an SDN controller, an OpenFlow virtual switch (OVS), and hosts connected to the OVS. The job of the control plane is to manage what and how data is being transmitted while the OVS listens to whatever the controller tells it to do. The controller manages the virtual switch by setting OpenFlow (OF) rules. Network admin can add These rules statically using the OpenFlow vSwitch command line tools or by writing scripts to instruct the controller to add rules according to particular situations. We use the latter for our DNS MTD implementation. OpenFlow rules have two fields that can be utilized to implement the MTD within DNS. They are a field called match and a field called actions. The match field is to match flows that have the defined parameters. In the MTD within DNS case, we match the flows that use UDP protocol, have a port number 53, and are sent from the host VM to one of the DNS servers. As the name suggests, the action field sets actions when a flow is matched with defined parameters. In the DNS MTD case, we set the actions to handle the responses from the backup DNS servers whenever the load balancing is applied. We utilize the Group rule to implement the load balancing between two servers. We use a SELECT Group rule that sets a bucket for each DNS server. We can declare a weight for each bucket. We declare a 50-50 weight for the two buckets in our implementation, which split the DNS traffic into half and load-balance them to two DNS servers. At the development phase, we used a Packet-In to trigger the monitoring task. We found this method introduced an inevitable latency on the first DNS packet after the Packet-In rule is installed. The reason for the latency is because the controller needs to receive a Packet-In message before installing the DNS request rule. After, we switch to set the DNS request rule as a default rule. This solution eliminates the latency.



\textbf{VM Automation Using Vbox}:
we implement automation using the VBox command line manager called "VBoxManage." It allows us to start and save the state of a VM, which is a good choice for implementing automation. We emulate a middleware environment that controls the start and stop of the VM. 

\subsection{Evaluation Metrics}
The following metrics are used to evaluate the performance of the proposed approach:
\begin{enumerate}
    \item Average Latency:
     The average of time required for a DNS server to respond to a host's request. This metric measures the DNS resolution with and without SDN and Ryu running when a flooding attack is undergoing. In normal use, the two DNS servers we created can have a fair average latency. What if one of them is under attack? Therefore, we are interested in the average latency when a DNS server is under attacked.
    \item Query Completed Rate:
    The proportion of DNS queries that a DNS server successfully resolves out of the total number of queries it receives within a certain period of time.
    This metric is obtained by using DNSperf. This Query Completed Rate reflects not only the performance of DNS servers but also the performance enhancement when SDN and Ryu is in use. In other words, we are interested in the Query Completed Rate when one of the DNS servers is under attacked. Again, we will mimic a flooding attack when obtaining this metric.
    \item Load-Balancing:
    Distribution of queries between primary and backup DNS servers. This metric aims to verify a balanced query volume allocation between these servers.
    This graph is to visualize the time when the load-balancing is triggered. The data points on the graph are obtained by the calculated packet rate in a two seconds time window. Since we set a 50-50 weight for the two buckets in the group rule respectively, this graph should display a drop, perhaps a half of the spike, in packet rate when the DNS traffic is load-balanced. 
\end{enumerate}

\subsection{Results}
\label{result}
This section presents an analysis of the outcomes and a comparison of the DNS server's performance with and without the proposed MTD approach.
%\subsubsection{DNSperf of DNS Server with SDN, Ryu, and Hping3}
Table \ref{table:3} displays the results for the proposed approach obtained using load-balancing through SDN and emulating a flooding attack using Hping3. We set a count of 10000 and a payload of 120 bytes for Hping3's DNS requests. We observed that the DNS packets sent by DNSperf have a average packet size of 28 bytes for requests and 70 bytes for responses. Additionally, we use randomly generated IP addresses to perform the flooding attack. For the DNSperf, we use fixed queries per second of 100000 and a duration of 20 seconds. The number of clients is variable to show the differences among the results. We construct the test case by running the DNSperf on the client machine first and then the Hping3 on the attacker machine. We aimed to emulate the situation where the client is doing normal DNS requests, and the attack comes in. We obtained each result by running ten tests with the same parameter and taking the average. All the results reach a query completed rate of around 99.93\% and a latency of around 1.093 ms. 

\begin{table}[ht]
\caption{Average Latency and Query Completion Rate of DNS servers with MTDNS}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
100000 & 125 & 20 & 99.94\% &1.114 \\ 
\hline
100000 & 250 & 20 & 99.93\% &1.048\\
\hline
100000 & 500 & 20 & 99.93\% & 1.119\\
\hline
\end{tabular}
%\vspace{-0.2in}
\label{table:3}
\end{table}
\vspace{0.1in}

%\subsubsection{DNSperf of DNS Servers with Hping3}
 Table \ref{table:2} shows the results for DNSperf of DNS Server without the proposed MTD approach to evaluate the performance of the proposed apporoach.
The result is obtained  using the same parameters and test case used in the previous Table \ref{table:3}.
%\subsubsection{Comparison}
The query completed rates in Table \ref{table:2} are less than the ones in Table \ref{table:3}, which indicates our proposed method can bring the query completed rate back to around 99.93 percent even though a flooding attack is undergoing. The average latencies in Table \ref{table:2} are higher than in Table \ref{table:3}, indicating that our proposed method can reduce the average latency when a flooding attack occurs by load-balancing the DNS traffic between two servers. The average latency increases and the query completion rate drops as the number of clients increases. This is because an increase in the number of clients raises traffic, which may result in delays owing to congestion, and additional queuing and processing time. 

\begin{table}[ht]
\caption{Average Latency and Query Completion Rate of DNS servers without MTDNS}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
100000 & 125 & 20 & 88.94\% & 3.428 \\ 
\hline
100000 & 250 & 20 & 88.72\% &4.213\\
\hline
100000 & 500 & 20 & 86.41\% &4.133 \\ 
\hline
\end{tabular}
%\vspace{-0.2in}
\label{table:2}
\end{table}


%\subsubsection{DNS Load-Balancing Results}
Figure \ref{fig:PacketRate} visualizes when the load-balancing between two servers happened. We use flow-based statistics instead of port-based statistics, so we use the default packet rate calculated from the default DNS request rule before the load-balancing job happens and the default DNS server bucket packet rate from the group rule. The zero of the blue line is because the DNSperf we ran on the client machine needs time to load the DNS traffic. The purpose of using DNSperf is to emulate a normal DNS traffic pattern. Before the first spike, the packet rate becomes stable, around 10000 per second. The spike indicates the packet rate exceeds the threshold. If the request rule has a spike shown on the graph, the traffic will be load-balanced between two DNS servers. That is where the group is created, and the group rule is applied to the OVS. The drop after the first spike indicates the start of the load-balancing job. The red line represents the MTD packet rate. It remains zero before the group rule is applied. Once the group rule is installed, we fetch the backup DNS server bucket packet count for the MTD packet rate calculation. When the group rule and the group are deleted, the packet rate becomes zeros again. That is where the zeros are on the red line. Those zeros represent the load-balancing job that is not activated. The two spikes on the graph are mitigated by using MTD. The first load-balancing kicked in at 26 seconds and took and got mitigated in around 2.187 seconds. The second load-balancing kicked in at around 80 seconds and got mitigated in around 2.059 seconds. We determined the times by finding the intersections between the blue line and the red line.

%\begin{table}[ht]
%\centering
%\begin{tabular}{ |c|c|c|c|c| }
%\hline
%QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
%\hline
%100000 & 125 & 20 & 100\% &1.414\\ 
%\hline
%100000 & 250 & 20 & 100\% &1.226\\
%\hline
%100000 & 500 & 20 & 100\% & 1.377\\ 
%\hline
%\end{tabular}
%\caption{DNSperf of DNS Servers}
%\vspace{-0.2in}
%\label{table:1}
%\end{table}







\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/load-balancing1.png}
\caption{Load balancing in MTDNS} 
\vspace{-0.1in}
\label{fig:PacketRate}
\end{figure}
\vspace{0.1in}

==> experiment-old.tex <==
\section{Evaluation}
\label{ex}
In this section, we introduce the experimental environment and setup that we use to implement our proposed methodology. These experiments are conducted using traditional DNS protocol in the topology shown in Figure \ref{fig:Structure}. The experimental metrics and the results are provided subsequently. The source code and scripts developed for the realization of this project are available on Git Hub \footnote{Gradresearch: Dns mtd,” Online, Dec 2023. [Online]. Available: https://github.com/Water-Meloon/GradResearch}.
%~\cite{github}.

\subsection{Setup Overview}
The hardware, operating system, OVS, and SDN, as well as the DNS server and structure details used in our experimental setup, are defined and described in this subsection.
%As part of our experimental setup, we define and describe our hardware, Operating System, OVS and SDN, and DNS traffic and structure details.

\textbf{Hardware and Operating System}: We have Dell Desktops with an i7 CPU with 20 cores, 32GB RAM, and 512GB SSD storage. For the SDN setup, we configure the Desktop as the OVS switch. By redirecting the network connection from OVS to the network stack to the actual Ethernet interface, we can create a structure shown in Figure \ref{fig:Structure}. Ubuntu server version 20.04.6 LTE is used as our operating system. 


\begin{figure}[h]
\centering
\includegraphics[width=.70\linewidth]{fig/topo1.pdf}
\caption{Experiment Topology} 
%\vspace{-0.1in}
\label{fig:Structure}
\end{figure}

%\textbf{Operating System}: We use Ubuntu server version 20.04.6 LTE as our operating system. %We use Ubuntu because installing OVS on Windows is tedious. On the contrary, we just need to use a couple of commands to finish the installation of OVS on Ubuntu. 

\textbf{OVS and SDN controller}: We use Open vSwitch version 2.13.8 and RYU as SDN controller for the experiment. The MTD logic is written directly in RYU. The controller's job is to continuously monitor DNS flows and write rules to respond to suspicious or simply increasing DNS requests and provide resilience. We write our logic directly for the controller instead of retrieving statistics from the API.

%\textbf{Vbox and VM Resource Allocation}:
%Upon further investigation, we find that Vbox starts a VM with high latency. This could be due to the fact that Vbox virtualizes the entire hardware infrastructure of the computer and allows users to install different operating systems on each VM they create. We allocate 2 GB RAM and 25 GB disk space to each VM. 

%Since we use VMs instead of containers, we ran into a situation in the test phase where VMs crashed and were aborted. So we realized that it is resource intensive to allocate ample storage space and CPU to the VMs. Therefore, we have allocated consistent and adequate resources to our infrastructure accordingly. Each VM setup are described as follows:
\textbf{Host VMs:} To emulate the situation where a legitimate user sends DNS requests to the default DNS server, an attacker overwhelms the default DNS server. We have created two VMs for this situation. VM Host 1 is for the client, and VM Host 2 is for the attacker. We use Hping3~\cite{hpingwiki} and DNSperf~\cite{dnsperf} on the attacker machine and the client machine.

\textbf{DNS Server VM:} We use the structure of BIND9~\cite{jinmei2006implementation} to implement our DNS servers as VNFs using VMs and VNF Manager. We set DNS servers as recursive resolvers. We use Virtualbox as a VM manager because it can connect VMs to virtual taps created on a virtual bridge. Since the DNS servers are VNFs, we install the two DNS servers (i.e., DNS resolvers) on two VMs managed by VNF Manager (i.e., Virtualbox). To do this, we create two virtual Ethernet adapters on our host machine, and two virtual DNS servers are connected to the OVS bridge via these two virtual taps. One of the DNS servers acts as a backup DNS resolver when needed. 

\textbf{Backup DNS VM:} As described in the previous section, the backup DNS VM helps the default DNS server unload DNS traffic when needed. We have two preset thresholds. One is used to trigger the start of the backup DNS server. Another is for forwarding traffic to the newly generated VNF (i.e., the backup DNS). The first threshold is calculated by taking half of the load balancing threshold. We start the backup server first to avoid the startup latency caused by the VM boot process. The flow of the backup DNS VM is that the backup server is started when the VM startup threshold is exceeded. When the critical traffic load threshold is exceeded, the DNS traffic between the two shared servers is established by an OpenFlow group rule.


\textbf{VM Automation Using Vbox}:
We implement automation using the VBox command line manager called "VBoxManage." It allows us to start and save the state of a VM, which is a good choice for implementing automation. We emulate a middleware environment that controls the starting and stopping of the VM.

\textbf{SDN and OpenFlow}: 
We use SDN capabilities to implement our MTD approaches for DNS defense. OpenFlow rules have two fields that can be used to implement MTD in DNS. These are a field called Match and a field called Actions. The Match field is used to match flows with the defined parameters. In the case of MTD within DNS, we match the flows that use the UDP protocol, have port number 53, and are sent from the host VM to one of the DNS servers. As the name suggests, the action field defines actions when a data flow is matched with defined parameters. In MTDNS, we set the actions with which the responses from the backup DNS servers are to be handled when the mitigation procedure is applied.

\textbf{Zone File Migration}: We use the master-slave DNS configuration (i.e., primary-secondary DNS) to migrate the zone file. The idea is that the master server can transfer its zone file to its slave servers. The slave servers cannot modify the zone file received from the master server, which is read-only. The zone file transfer can be implemented by configuring a DNS server as the master server and the "allow transfer" option in the DNS server configuration file. This option allows the admin to specify which IP address or IP range the zone file is going to. The admin may also set the "also-notify" option to notify the slave servers that the zone file is reloaded. This option requires the slave servers to set the "allow-notify" option to accept the notification from the master server properly.



\subsection{Evaluation Metrics}
The following metrics are used to evaluate the performance of the proposed approach:
\begin{enumerate}
    \item \textbf{Average Latency:}
     The average time required for a DNS server to respond to a host's requests. This metric measures the DNS resolution with and without the SDN Controller (i.e., Ryu running) when a flooding attack occurs. 
     
    \item \textbf{Query Completion Rate:}
    This metric measures the proportion of DNS queries that a DNS server successfully resolves out of the total number of queries it receives within a certain period of time.
    This metric is obtained by using DNSperf \cite{dnsperf}.
    
    \item \textbf{Attack Mitigation Time:} This metric measures the time taken by MTDNS to respond and mitigate a sudden spike in incoming requests indicative of a potential attack. The data is derived by plotting the rate of network traffic in DNS servers while MTDNS is in operation, which demonstrates the time when the new VNF (i.e., backup DNS server) is initialized, and the network traffic is shared between the default and backup server. 
\end{enumerate}



\subsection{Results}
\label{result}

This section analyses the results and compares the performance of the DNS server with and without the proposed MTDNS approach. Our setup consists of a client, attackers, and DNS servers, as shown in Figure \ref{fig:Structure}. We aim to emulate the situation where the client makes normal DNS requests, and the attack begins. We construct the test case by first running the DNSperf on the client machine and then the Hping3 on the attackers' machine. The DNS packets sent by clients using DNSperf have an average packet size of 28 bytes for requests and 70 bytes for responses. We also use a fixed client count of 125 and a duration of 20 seconds. The number of queries per second (QPS) varies to account for the impact of traffic volume on the results. For Hping3, we use randomly generated IP addresses to perform the DNS flooding attack. We set a payload of 120 bytes and a QPS of 80000 for the DNS requests of Hping3. We obtain average values for each result by running ten tests with the same parameters and taking the average. 

Table \ref{table:2} shows the results for DNSperf of DNS Server without the proposed MTD approach. The table shows that average latency increases, and the query completion rate drops as the number of clients increases. This is because increasing the number of clients raises traffic, which may result in delays owing to congestion and additional queuing and processing time. According to the table, without MTDNS, we obtain 92.33\% as the highest query completion rate. The effect of a DNS flooding attack becomes more visible with higher QPS, resulting in a 77.35\% query completion rate and an average latency of 4.579ms.
 

\begin{table}[ht]
\caption{Average Latency and Query Completion Rate of DNS servers without MTDNS}
\centering
\begin{tabular}{ |c|c|c|c| }
\hline
QPS  &  Query Completed & Avg Latency(ms) \\
\hline
5000  &  92.33\% & 3.665 \\ 
\hline
10000  &  91.14\% & 3.303\\
\hline
15000  &  77.35\% & 4.579 \\ 
\hline
\end{tabular}
%\vspace{-0.1in}
\label{table:2}
\end{table}

Table \ref{table:3} shows the results for the MTDNS (i.e., the proposed approach) obtained with SDN and emulating a flooding attack with Hping3. The results show that our proposed method can bring the query fulfillment rate back to about 99.8\%. There is also an interesting result we observe in this test, which is the increasing query completion by the increased QPS. We believe it is due to the fact that the average latency 


\begin{table}[ht]
\caption{Average Latency and Query Completion Rate of DNS servers with MTDNS}
\centering
\begin{tabular}{ |c|c|c|c| }
\hline
QPS &  Query Completed & Avg Latency(ms) \\
\hline
5000   & 99.68\% &0.966 \\ 
\hline
10000   & 99.79\% &1.006\\
\hline
15000 & 99.86\% & 1.005\\
\hline
\end{tabular}
\vspace{-0.1in}
\label{table:3}
\end{table}

Figure \ref{fig:PacketRate} visualizes alleviating the load on the DNS servers when the MTDNS is activated. We use the default packet rate calculated from the default DNS request rule before the MTDNS functions execution and the default DNS server bucket packet rate from the group rule. The purpose of using DNSperf is to emulate a regular DNS traffic pattern. Before the first spike, the packet rate becomes stable, around 10000 QPS. The spike indicates that the packet rate exceeds the threshold to trigger VNF Manager. If the request rule has a spike shown on the graph, the traffic will be transmitted and divided between two DNS servers. That is implemented and tested through the OF group that is applied to the OVS. The drop after the first spike indicates the start of the MTDNS, which has mitigated the attack and provided resiliency. The red line represents the packet rate for the backup DNS server. It remains zero before the group rule is applied (i.e., VNF has not been needed). Once the group rule is installed, we fetch the backup DNS server bucket packet count for the MTD packet rate calculation. When the group rule and the group are deleted, the packet rate becomes zeros again. That is where the zeros are on the red line. Those zeros represent that the backup DNS server is not needed, and the resources are deallocated. The two spikes on the graph are mitigated by using MTD. The initial MTDNS detection and activation take place at the 30-second mark, and the traffic is mitigated within around 2.1 seconds. The second mitigation is initiated at approximately the 80th second, resulting in mitigation in approximately 2.3 seconds. These times are determined by finding the exact values of the data at the intersections between the blue and red lines.

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/load_balancing3.png}
\caption{Network Traffic in DNS Servers while MTDNS is running} 
%\vspace{-0.1in}
\label{fig:PacketRate}
\end{figure}

==> experimental-old.tex <==
\section{Evaluation}
\label{ex}
In this section, we introduce the experimental environment and setup that we use to implement our proposed methodology. These experiments are conducted using traditional DNS protocol in the topology shown in Figure \ref{fig:Structure}. The experimental metrics and the results are provided subsequently. The source code and scripts developed for the realization of this project is available on github~\cite{github}.

\subsection{Setup Overview}
The hardware, operating system, OVS and SDN, as well as the DNS server and structure details used in our experimental set up, are defined and described in this subsection.
%As part of our experimental setup, we define and describe our hardware, Operating System, OVS and SDN, and DNS traffic and structure details.

\textbf{Hardware and Operating System}: We have Dell Desktops with an i7 CPU with 20 cores, 32GB RAM, and 512GB SSD storage. For the SDN setup, we configure the Desktop as the OVS switch. By redirecting the network connection from OVS to the network stack to the actual Ethernet interface, we can create a structure shown in Figure \ref{fig:Structure}. Ubuntu server version 20.04.6 LTE is used as our operating system due to its open-source nature, networking capabilities, and compatibility with a wide range of security tools. %The experiment is tested under a network throughput of 4.75 Gbps. 


\begin{figure}[h]
\centering
\includegraphics[width=.60\linewidth]{fig/topo.pdf}
\caption{Experiment Topology} 
\vspace{-0.1in}
\label{fig:Structure}
\end{figure}

%\textbf{Operating System}: We use Ubuntu server version 20.04.6 LTE as our operating system. %We use Ubuntu because installing OVS on Windows is tedious. On the contrary, we just need to use a couple of commands to finish the installation of OVS on Ubuntu. 

\textbf{OVS and SDN controller}:
We use Open vSwitch version 2.13.8, and RYU as the SDN Controller for the experiment. The MTD logic is written directly to RYU. The controller's job is to continually monitor the DNS flows and write rules to respond to and provide resiliency against suspicious or just increasing DNS requests. We write our logic directly applicable to the controller instead of fetching statistics from API.

\textbf{Vbox and VM Resource Allocation}:
As a further investigation, we find out that Vbox starts a VM with high latency. This might be because Vbox virtualizes the whole computer hardware infrastructure and allows users to install different OSs on each VM they have created. Yet, Docker virtualizes the kernel OS, which allows OSs that share the same kernel as the host to be virtualized. For example, a user uses Ubuntu as the host OS and may only be able to install OSs from the Linux distribution in the Docker containers. Docker is meant to provide a lightweight solution using kernel virtualization. We plan using Docker to create containers and connect them to the OVS we have already created. This can be achieved via ovs-docker utility that needs to be downloaded from the OVS GitHub page~\cite{Openvswitch}. The difficulty of using Docker is that we need to use Kubernetes as the orchestrator of the containers we have created. One might think of the role of Kubernetes as the vSphere of VMs. Using Kubernetes with SDN causes additional complexity in the implementation, and we need to use CNI (Container Network Interface) to create an overlay network. This is called OVN (Open Virtual Network). Considering the implementation complexity, we use VBox's command line management tool to achieve starting VMs on the fly. We allocate each VM with 2 GB of RAM and 25 GB of storage. Since we use VMs instead of containers, we ran into a situation where VMs crashed and were aborted during the testing phase. Thus, we realized that it is resource-consuming to allocate ample storage space and CPU for the VMs. Therefore, we allocate even and reasonable resources according to our infrastructure. Each VM setup are described as follows:
\begin{itemize}
    \item Host VMs: In order to emulate the situation where a legitimate user sends DNS requests to the default DNS server, an attacker bombards the default DNS server. We created two VMs dedicated to this situation. VM Host 1 is for the client, and VM Host 2 is for the attacker. We use Hping3~\cite{hpingwiki} and DNSperf~\cite{dnsperf} on the attacker machine and the client machine.
    \item DNS Server VM: We use the BIND9~\cite{jinmei2006implementation} structure to implement our DNS servers as VNFs utilizing VMs and VNF Manager. We set DNS servers as the recursive resolvers. We use Virtualbox as the VM manager since Virtualbox can connect VMs to virtual taps created on a virtual bridge. Virtualbox also provides a command line management tool called VBoxManage, which is useful in terms of starting or stopping a VM. In terms of DNS servers, since they are VNFs, we install the two DNS servers (i.e., DNS resolvers) on two VMs that VNF Manager (i.e., Virtualbox) manages. In order to do this, we create two virtual Ethernet adapters on our host machine, and two virtual DNS servers are connected to the OVS bridge through these two virtual taps on the OVS bridge. One of the DNS servers works as a backup DNS resolver whenever it is needed. 
    \item Backup DNS VM: As described in the previous section, the backup DNS VM helps the default DNS server unload DNS traffic whenever needed. We have two pre-set thresholds. One is for triggering the startup of the backup DNS server. Another one is for forwarding the traffic to the newly generated VNF (i.e., backup DNS). The first threshold is calculated by taking the half of the load-balancing threshold. We start the backup server first, which can defeat the startup latency introduced by the VM booting process. The flow of the backup DNS VM is that the backup server is started when the VM startup threshold is exceeded. When the critical traffic load threshold is exceeded, the DNS traffic between the divided two servers is set up by an OpenFlow group rule.
\end{itemize} 

\textbf{VM Automation Using Vbox}:
We implement automation using the VBox command line manager called "VBoxManage." It allows us to start and save the state of a VM, which is a good choice for implementing automation. We emulate a middleware environment that controls the start and stop of the VM. 

\textbf{SDN and OpenFlow}: 
We utilize SDN capabilities to implement our MTD approaches for the DNS defense. OpenFlow rules have two fields that can be utilized to implement the MTD within DNS. They are a field called match and a field called actions. The match field is to match flows that have the defined parameters. In the MTD within the DNS case, we match the flows that use UDP protocol, have a port number 53, and are sent from the host VM to one of the DNS servers. As the name suggests, the action field sets actions when a flow is matched with defined parameters. In the MTDNS, we set the actions to handle the responses from the backup DNS servers whenever the mitigation procedure is applied. We utilize the Group rule to implement the mitigation procedure from default server to backup server. We use a SELECT Group rule that sets a bucket for each DNS server. We can declare a weight for each bucket. We declare a 50-50 weight for the two buckets in our implementation, which split the DNS traffic into half and load-balance them to two DNS servers. We set the DNS request rule as a default rule in the beginning of the experiments. 

%During the development phase, we used a Packet-In to trigger the monitoring task. We found this method introduced an inevitable latency on the first DNS packet after the Packet-In rule was installed. The reason for the latency is that the controller needs to receive a Packet-In message before installing the DNS request rule. After that, we switch to setting the DNS request rule as a default rule. This solution eliminates the latency.


\textbf{Zone File Migration}:
We consider using a shared folder to emulate a cloud-like environment for performing zone file transfer. Yet, we find that the master-slave DNS server configuration is less complex in configuration, and this utility comes with the BIND9 server. We use the master-slave DNS configuration or the primary-secondary DNS configuration to migrate the zone file. The idea is that the master server can transfer its zone file to its slave servers. That means that slave servers do not need a zone file configured. The slave servers cannot modify the zone file received from the master server, which is read-only. We find that the zone file transfer is performed using normal traffic, so we set a flow rule to direct the normal traffic, as mentioned. The zone file transfer can be implemented by configuring a DNS server as the master server and the "allow transfer" option in the DNS server configuration file. This option allows the admin to specify which IP address or IP range the zone file is going to. The admin may also set the "also-notify" option to notify the slave servers that the zone file is reloaded. This option requires the slave servers to set the "allow-notify" option to accept the notification from the master server properly.
%named.conf.local file







\subsection{Evaluation Metrics}
The following metrics are used to evaluate the performance of the proposed approach:
\begin{enumerate}
    \item \textbf{Average Latency:}
     The average time required for a DNS server to respond to a host's requests. This metric measures the DNS resolution with and without the SDN Controller (i.e., Ryu running) when a flooding attack occurs. In normal use, the DNS server we created and run would have a relatively reasonable average latency. What if one of them is under attack? Therefore, we are primarily interested in determining the average latency when a DNS server is under attack.
     
    \item \textbf{Query Completion Rate:}
    This metric measures the proportion of DNS queries that a DNS server successfully resolves out of the total number of queries it receives within a certain period of time.
    This metric is obtained by using DNSperf \cite{dnsperf}. This query completion rate reflects not only the performance of DNS servers but also the performance enhancement when SDN and NFV are in employed. In other words, we are interested in the query completed rate when one of the DNS servers is under attack. We mimic a flooding attack when obtaining this metric.
    
    \item \textbf{Attack Mitigation Time:} This metric measures the time taken by MTDNS to respond and mitigate a sudden spike in incoming requests indicative of a potential attack. The data is derived by plotting the rate of network traffic in DNS servers while MTDNS is in operation, which demonstrates the time when the new VNF (i.e., backup DNS server) is initialized, and the network traffic is shared between the default and backup server. The data points on the plot are obtained by the calculated packet rate in a two-second time window. Since we set a 50-50 weight for the two buckets in the group rule respectively, this graph should display a drop, perhaps half of the spike, in packet rate when the DNS traffic is redirected. 
    %\item Load-Balancing:
    %This metric displays the distribution of queries between primary and backup DNS servers. This metric aims to verify a balanced query volume allocation between these servers.
    %This graph is used to visualize the time when the new VNF (i.e., backup DNS server) is initialized, and the network traffic is divided between them. The data points on the graph are obtained by the calculated packet rate in a two-second time window. Since we set a 50-50 weight for the two buckets in the group rule respectively, this graph should display a drop, perhaps half of the spike, in packet rate when the DNS traffic is load-balanced. 
    
\end{enumerate}

\subsection{Results}
\label{result}
This section presents an analysis of the outcomes and a comparison of the DNS server's performance with and without the proposed MTDNS approach.
%\subsubsection{DNSperf of DNS Server with SDN, Ryu, and Hping3}

Our setup consists of a client, attackers, and DNS servers, as depicted in Figure \ref{fig:Structure}. We aim to emulate the situation where the client is doing regular DNS requests, and the attack starts. We construct the test case by running the DNSperf on the client machine first and then the Hping3 on the attacker machine. The DNS packets sent by clients using DNSperf have an average packet size of 28 bytes for requests and 70 bytes for responses. Additionally, we use a fixed client number of 125 and a duration of 20 seconds. The number of queries per second (QPS) varies to reflect the impact of traffic volume on results. For Hping3, we use randomly generated IP addresses to perform the DNS flooding attack. We set a payload of 120 bytes, and the QPS is 80000 for Hping3's DNS requests. We obtain averages of each result by running ten tests with the same parameter and taking the average. 

%As the first experiment, we run different number of clients with a query count per second of 100.000 and a payload of 120 bytes for Hping3's DNS requests without any MTD approach employed.
Table \ref{table:2} shows the results for DNSperf of DNS Server without the proposed MTD approach. The table shows the average latency increases, and the query completion rate drops as the number of clients increases. This is because increasing the number of clients raises traffic, which may result in delays owing to congestion and additional queuing and processing time. According to the table, without MTDNS, we obtain 92.33\% as the highest query completion rate. The effect of a DNS flooding attack becomes more visible with higher QPS, resulting in a 77.35\% query completion rate and an average latency of 4.579ms.
 

\begin{table}[ht]
\caption{Average Latency and Query Completion Rate of DNS servers without MTDNS}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS  & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
5000  & 20 & 92.33\% & 3.665 \\ 
\hline
10000  & 20 & 91.14\% & 3.303\\
\hline
15000  & 20 & 77.35\% & 4.579 \\ 
\hline
\end{tabular}
%\vspace{-0.2in}
\label{table:2}
\end{table}



Table \ref{table:3} displays the results for the MTDNS (i.e., proposed approach) obtained employing SDN and emulating a flooding attack using Hping3. The results indicate that our proposed method can bring the query completed rate back to around 99.8\% % even though a flooding attack occurs. The average latencies in Table \ref{table:2} are at least 2ms higher than in Table \ref{table:3}, indicating that our proposed method can also reduce the average latency when a flooding attack occurs. We observe that the query completion rate and average latency in Table \ref{table:3} are more consistent and stable than Table \ref{table:2}, which implies the resiliency and reliability of the proposed solution. Furthermore, we can see the effectiveness of the MTDNS most with the higher QPS on Query Completion rate with a 22.51\% % increase in query completion and a 3.128 reduction in average latency. 

%All the results reach a query completed rate of nearly 100\% and a latency of around 1.093 ms. 
%The result is obtained  using the same parameters and test case used in the previous Table \ref{table:2}.




\begin{table}[ht]
\caption{Average Latency and Query Completion Rate of DNS servers with MTDNS}
\centering
\begin{tabular}{ |c|c|c|c|c| }
\hline
QPS & Time(s) & Query Completed & Avg Latency(ms) \\
\hline
5000  & 20 & 99.68\% &0.966 \\ 
\hline
10000  & 20 & 99.79\% &1.006\\
\hline
15000 & 20 & 99.86\% & 1.005\\
\hline
\end{tabular}
%\vspace{-0.2in}
\label{table:3}
\end{table}
\vspace{0.1in}



%\subsubsection{DNS Load-Balancing Results}
%Figure \ref{fig:PacketRate} visualizes when the MTDNS got applied, and the load of the DNS servers got eased. 
Figure \ref{fig:PacketRate} visualizes alleviating the load on the DNS servers when the MTDNS is activated. We use the default packet rate calculated from the default DNS request rule before the MTDNS functions execution and the default DNS server bucket packet rate from the group rule. The purpose of using DNSperf is to emulate a regular DNS traffic pattern. Before the first spike, the packet rate becomes stable, around 10000 QPS. The spike indicates that the packet rate exceeds the threshold to trigger VNF Manager. If the request rule has a spike shown on the graph, the traffic will be transmitted and divided between two DNS servers. That is implemented and tested through the OF group that is applied to the OVS. The drop after the first spike indicates the start of the MTDNS, which has mitigated the attack and provided resiliency. The red line represents the packet rate for the backup DNS server. It remains zero before the group rule is applied (i.e., VNF has not been needed). Once the group rule is installed, we fetch the backup DNS server bucket packet count for the MTD packet rate calculation. When the group rule and the group are deleted, the packet rate becomes zeros again. That is where the zeros are on the red line. Those zeros represent that the backup DNS server is not needed, and the resources are deallocated. The two spikes on the graph are mitigated by using MTD. The initial MTDNS detection and activation take place at the 30-second mark, and the traffic is mitigated within around 2.1 seconds. The second mitigation is initiated at approximately the 80th second, resulting in mitigation in approximately 2.3 seconds. These times are determined by finding the exact values of the data at the intersections between the blue and red lines.

%The first MTDNS detection and trigger occur at 30 seconds, and the traffic is mitigated in around 2.1 seconds. The second load-balancing is activated at around 80 seconds and cause mitigation in around 2.3 seconds. We determined the times by finding the exact values of the data at the intersections between the blue line and the red line.

%\begin{table}[ht]
%\centering
%\begin{tabular}{ |c|c|c|c|c| }
%\hline
%QPS & clients & Time(s) & Query Completed & Avg Latency(ms) \\
%\hline
%100000 & 125 & 20 & 100\% &1.414\\ 
%\hline
%100000 & 250 & 20 & 100\% &1.226\\
%\hline
%100000 & 500 & 20 & 100\% & 1.377\\ 
%\hline
%\end{tabular}
%\caption{DNSperf of DNS Servers}
%\vspace{-0.2in}
%\label{table:1}
%\end{table}





%figure not clear? maybe redraw?? 

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/load_balancing3.png}
\caption{Network Traffic in DNS Servers while MTDNS is running} 
\vspace{-0.1in}
\label{fig:PacketRate}
\end{figure}
\vspace{0.1in}

==> futureWork.tex <==
\section{Future Work}
\label{future_work}
During the experiment, we found that VMs are not the ideal implementation for vDNS. The startup of VMs introduces a unacceptable latency when we try to implement fast DNS server startup. We will switch to Docker environment in the future for fast DNS server startup. Kubernetes is the orchestrator for Docker containers, and it is compatible with SDN by creating a OVN. Therefore, Docker environment is more suitable to our proposed methodology. We consider moving to Docker environment and performing our experiment in a larger network topology to collect more reliable results. 
The scale of our experiment is small. We will move our methodology to Mininet and perform a large scale testing on Mininet. 
We briefly mentioned about the detection logic for DNS amplification attacks, but we did not go deep into it. We will consider MTD for DNS amplification attacks in the future.




==> intro.tex <==
\section{Introduction}

DNS (Domain Name System) is the system that maps human-readable domain names (e.g., www.mywebsite.com) to IP addresses (e.g., 192.168.0.1). It works by having a hierarchical structure of servers, where each server is responsible for a portion of the domain name space. When a client wants to resolve a domain name, it sends a query to a DNS resolver, which then contacts authoritative servers from the top of the hierarchy down until it finds the IP address for the requested domain name.

%However, as practical as it is, DNS has some potential vulnerabilities. For example, DNS spoofing, where an attacker intercepts a DNS query and returns a false IP address, redirecting traffic meant for a legitimate website to a malicious one. Another vulnerability is cache poisoning, where an attacker tricks a DNS resolver into caching a false IP address for a domain name, again leading to traffic being redirected to a malicious website. To address these vulnerabilities, this research involves implementing a DNS server on a virtualized environment using NFV and SDN concepts. Both virt-manager and virsh are used as tools to achieve NFV capabilities. Open vSwitch will be used to connect the virtual machines and create virtual networks, with some virtual machines representing DNS servers and others representing nodes in the network.

Traditionally, the DNS resolver can be located within and operated by an Internet Service Provider (ISP), a mobile carrier, a WIFI network, or another third party. In this work, we consider running a local DNS resolver as a Virtual Network Function (VNF), which small enterprises can also employ \cite{infoblox}. In other words, we consider an edge DNS service, which replicates consumer-based networking equipment and offers numerous benefits to organizations. With Edge DNS, a distributed network of servers can efficiently and quickly resolve DNS queries \cite{callejo2019measuring}. By doing so, users receive responses from the closest available server, thereby reducing latency and improving performance. By managing DNS records and configurations in real-time, Edge DNS provides organizations with greater flexibility and control. As well as advanced features such as traffic management, load balancing, and security measures like DDoS protection, edge DNS is a valuable tool for ensuring online service availability and security. Ultimately, edge DNS provides substantial benefits for organizations seeking to enhance the speed, reliability, security, and flexibility of their DNS infrastructures.


The DNS protocol has received much attention recently by different organizations and academia due to its lack of encryption or integrity in the traditional DNS protocol messages. For security improvements, a few of the popular protocols are being proposed and currently in use by some DNS servers are DNSSEC (DNS Secure), DNS over Transport Layer Security (TLS), DNS over Hypertext Transfer Protocol Secure (HTTPS), and DNS over QUIC (DoQ).
It is crucial to note that DNS security protocols have their advantages and disadvantages and varying performances depending on the network conditions and hardware resources available. As part of this paper, we perform a comprehensive test that any enterprise could use to decide which DNS security protocol to employ. We measure response times, setup times, and network traffic under various conditions to determine which protocol performs better. Some DNS security protocols may provide more robust security but require more resources and complicated configuration, while others may offer better privacy and perform better in certain circumstances. Organizations and consumers can determine which protocol to use during comparative testing based on their specific needs through the testing platform, evaluation metrics, and results we present in this paper.


==> lcn/intro2.tex <==
\section{Introduction}

In the constantly growing interconnected world of cyberspace, the Domain Name System (DNS) serves a critical part by enabling the conversion of human-readable domain names (e.g., www.example.com) into machine-readable IP addresses (e.g., 192.168.0.1). The significance and visibility of DNS make it a primary target for malicious cyber-attacks, specifically Distributed Denial of Service (DDoS) attacks. In a DDoS attack, by deliberately disrupting DNS servers, attackers impair the machines' capacity to establish a connection with a website, consequently rendering websites inaccessible to users. This disruption results in revenue losses, damaged reputations, and user dissatisfaction, which aligns with the attackers' goal of causing chaos for their targets. DDoS attacks are occasionally used as a diversion from cybersecurity operations during other illegal activities, such as network intrusion or data theft. Moreover, a significant concern regarding IoT devices is that they are vulnerable to being transformed into botnets, which can be utilized for launching DDoS attacks~\cite{hayat2022ml}. This vulnerability originates from inherent weaknesses, such as the prevalence of weak or default passwords and inadequate security configurations, which grant unauthorized access to management systems and administrative controls. Based on Cloudflare's third DDoS threat report of 2023~\cite{Yoachimik_2023}, DNS-based DDoS attacks emerged as the predominant form of attack, constituting over 47\% of the total attacks. This signifies a 44\% surge in comparison to the preceding quarter of the year. 

Researchers are constantly involved in the pursuit of new methods and strategies to address and minimize the impact of DDoS attacks effectively. In the last few years, researchers have shown keen interest in Software-Defined Networking (SDN)~\cite{bawany2017ddos} and Network Functions Virtualization (NFV)~\cite{yi2018comprehensive, han2015network} based solutions for addressing DDoS attacks in DNS. SDN functionalities, including traffic analysis, dynamic packet forwarding rule configuration, and global network views, are widely utilized and leveraged to mitigate the challenges posed by DDoS attacks. At the same time, the NFV facilitates resource allocation and on-demand function instantiation flexibility and introduces new possibilities for mitigating DDoS attacks~\cite{zhou2017applying}. In addition, the Moving Target Defense (MTD)~\cite{cho2020toward} technique has emerged as a promising approach in the field of network security~\cite{huang2021trend}. The idea of MTD involves the dynamic alteration of network configuration and behavior. Its purpose is to enhance uncertainty and seeming complexity for potential attackers, consequently decreasing their chances of success and raising the costs associated with their probing and attack activities. 


Current approaches primarily combat DDoS attacks against DNS protocol and infrastructure by discarding or blocking suspicious traffic~\cite{xing2016defense, abou2020bringing, sagatov2023countering, gupta2018mitigating}. Certain solutions prioritize rerouting the traffic with network orchestration, which can result in a higher computational burden due to the added complexity of managing and coordinating multiple components, such as data centers and servers, within an orchestrated workflow~\cite{fayaz2015bohatei}. Additionally, these solutions may not be effective if the available server resources are exhausted. 
These works assume or try to understand and estimate the DNS clients' behavior as either malicious or legitimate \cite{nesary2022vdns}.
Yet, how the defense mechanisms should work has not been investigated when we do not have clear and concise knowledge of the clients. Therefore, these methods rely on the detection of malicious traffic vs. legitimate, which carries the inherent risk of legitimate packet loss if the detection mechanism lacks accuracy. 


%In this paper, we propose a solution named \textit{MTDNS} that utilizes NFV with MTD techniques to mitigate DDoS attacks in the DNS. More specifically, the focus is on defending against flooding attacks by redirecting DNS traffic to a backup DNS server upon detecting an change of the network traffic pattern. The proposed approach offers increased flexibility for real-time and adaptable modifications, while simultaneously reducing computational burden and minimizing the risk of legitimate packet loss. The contributions of this paper can be summarized as follows: (i) A resilient DDoS Defense mechanism that utilizes MTD is designed for DNS in general SDN environments; (ii) The proposed approach is implemented as a SDN application  that operates on a widely used SDN controller called RYU~\cite{ali2018performance}; (iii) This system is evaluated in a real-world setup, and the experimental outcomes demonstrate an almost perfect success rate of nearly 100\% in resolving DNS queries and a significant improvement in average latency.
In this paper, we propose a solution named \textit{MTDNS} that utilizes NFV with MTD techniques to mitigate DDoS attacks against the DNS servers. More specifically, the focus is on defending against flooding attacks by redirecting DNS traffic to a backup DNS server upon detecting a change in the network traffic pattern. The proposed approach offers increased flexibility for real-time and adaptable modifications while simultaneously reducing the computational burden and minimizing the risk of legitimate packet loss. The contributions of this paper can be summarized as follows: (i) A resilient DDoS Defense mechanism that utilizes MTD is designed for DNS in general SDN environments; (ii) The proposed approach is implemented as an SDN application; (iii) This system is evaluated in a real-world setup.


The subsequent sections of the paper are structured in the following manner: Section~\ref{related_work} presents a concise overview of the existing literature on strategies for mitigating DDoS attacks in the DNS. In Section~\ref{pre} the preliminary components related to the proposed solution are addressed and discussed. Subsequently, the proposed approach is introduced in Section~\ref{solution}. Section~\ref{ex} depicts the experimental setup and present the findings of our evaluation. Finally, Section~\ref{conclusion} concludes the paper via thorough discussion and consideration of future research endeavors.



%In the constantly growing interconnected world of cyberspace, the Domain Name System (DNS) serves a critical part by enabling the conversion of human-readable domain names (e.g., www.example.com) into machine-readable IP addresses (e.g., 192.168.0.1). The significance and visibility of DNS make it a primary target for malicious cyber attacks, specifically Distributed Denial of Service (DDoS) attacks. In DDoS attack, by deliberately disrupting DNS servers, attackers impair the machines' capacity to establish a connection with a website, consequently rendering websites inaccessible to users. This disruption results in revenue losses, damaged reputations, and user dissatisfaction, which aligns with the attackers' goal of causing chaos on their targets. DDoS attacks are occasionally used as a diversion from cybersecurity operations during other illegal activities, such network intrusion or data theft. Moreover, a significant concern regarding IoT devices is that they are vulnerable to being transformed into botnets, which can be utilized for launching DDoS attacks. This vulnerability originates from inherent weaknesses, such as the prevalence of weak or default passwords and inadequate security configurations, which grant unauthorized access to management systems and administrative controls. Based on Cloudflare's third DDoS threat report of 2023 ~\cite{Yoachimik_2023}, DNS-based DDoS attacks emerged as the predominant form of attack, constituting over 47\% of the total attacks. This signifies a 44\% surge in comparison to the preceding quarter of the year. 

% Researchers are constantly involved in the pursuit of new methods and strategies to effectively address and minimize the impact of DDoS attacks. In the last few years, researchers have shown keen interest in Software-Defined Networking (SDN) and NFV Network Functions Virtualization (NFV) based solutions for addressing DDoS attacks in DNS. These solutions primarily focus on mitigating amplification and flooding attacks, which are commonly observed in such attacks. In addition, the Moving Target Defense (MTD) technique has emerged as a promising approach in the field of network security~\cite{huang2021trend}. The idea of MTD involves the dynamic alteration of network configuration and behavior. Its purpose is to enhance uncertainty and seeming complexity for potential attackers, consequently decreasing their chances of success and raising the costs associated with their probing and attack activities. 

% Current approaches primarily combat DDoS attacks by either discarding suspected packets or isolating the nodes under suspicion. However, these methods carry the inherent risk of legitimate packet loss if the detection mechanism lacks accuracy. Certain solutions prioritize the network orchestration, even if it results in higher computing burden.

% To solve these problems, in this study, we propose a solution that utilizes SDN and NFV with MTD techniques to mitigate DDoS attacks in the DNS. More specifically, the focus is on defending against flooding attacks by redirecting traffic upon detecting an attack. The proposed approach offers increased flexibility for real-time and adaptable modifications, while simultaneously reducing computational burden and minimizing the risk of legitimate packet loss. 

% The subsequent sections of the paper are structured in the following manner: the preliminary components of the study are addressed in the next section. A concise overview of the existing literature on strategies for mitigating DDoS attacks in the DNS is provided afterwards. Then, we propose an approach for mitigating DDoS attacks in the DNS by employing MTD techniques and SDN. Subsequently, we proceed to depict the experimental setup and then present the findings of our evaluation. Finally, via thorough discussion and consideration of future research endeavors, we conclude the paper.


==> lcn/related.tex <==
\section{Related Work}
\label{related_work}
In recent years, the attention of researchers has been captured by SDN-based solutions for combating DDoS attacks against DNS, which aim to mitigate such attacks, predominantly encompassing flooding and amplification attacks. The literature on this domain varies, with some studies concentrating on detection, some on mitigation, and a few addressing both. The literature falls within this spectrum and can be categorized into detection strategies and mitigation strategies. The key phases of DDoS mitigation include detection and response phases, and we refer to the solutions that involve response as mitigation strategies in this paper. 
%While detection methods remain relevant, our research primarily contributes to advancing mitigation strategies. However, the process of detecting and minimizing the attacks poses significant challenges due to a variety of factors, including the precision of detection and, subsequently, the precision of mitigation. %The related works of this study can be categorised into detection strategies and mitigation strategies. 

\subsection{Detection Strategies}
Detection strategies entail monitoring patterns in traffic to identify attacks. This is vital to defending DNS against DDoS attacks because the mitigation depends on the output of this phase, and inaccuracies can have an immediate impact on users. The WisdomSDN~\cite{abou2020bringing} proposes the technique derived from the MTD, involves mapping between DNS request and response as well as utilizes the Bayes classifier to identify attacks based on entropy analysis. Another machine learning-based amplification attack detection scheme is presented in~\cite{chen2017detecting} that incorporates additional hardware referred to as a detecting agent connected to the OpenFlow switch that computes feature vectors of the flows and uses an SVM classifier to detect the attack. However, it can increase the overall cost in terms of equipment and overhead. The threat model of the paper~\cite{ahmed2017mitigating} includes both flooding and amplification attacks, and implements a Dirichlet process mixture model (DPMM) clustering algorithm to detect attack flows based on network statics in OpenFlow switches collected by the controller periodically. 
Xing et al.~\cite{xing2016defense} present a solution that detects DNS amplification attacks using packet rate and entropy calculation. While minimal resources are evident for this solution as it refrains from employing machine learning, the precision of detection can be lower with a constant threshold. A different amplification attack detection approach is proposed by Aizuddin et al.~\cite{aizuddin2017dns} that mainly matches the DNS request ID with the response to ensure that the DNS response is legitimate. 
Kim et al.~\cite{kim2017preventing} describes a DNS amplification attack mitigation system that can identify orphan DNS responses using a one-to-one strict mapping scheme between DNS requests and responses at OpenFlow switch and controller and drop these responses to mitigate attack. Gupta et al.~\cite{gupta2019dns} propose a solution that involves a shareable SDN barrier using a shared bloom filter through OpenFlow switch among all ISP connections of an organization to detect DNS amplification attack where legitimate DNS requests are added to the bloom filter, and DNS responses passing through the network are checked against it. If a response packet hashes any bit that is set to 0 in the bloom filter, it indicates the packet as illegitimate and dropped. A two-phased detection method for DNS amplification attacks called YASARA~\cite{ozdinccer2019sdn} is proposed that detects attacks by monitoring the ratio of DNS response size to the corresponding request and DNS client's hop count variation. When one of these values exceeds the threshold, the attack is mitigated by dropping all the responses of the corresponding DNS. On the other hand, Lyu et al.~\cite{lyu2021hierarchical} address the issue of DNS attacks on enterprise networks, utilizing trained and anomaly-based detection models to identify flooding attacks and scans from external sources of attacks instead of victims. They introduce a  hierarchical and dynamic graph data structure for scalable monitoring to find the key attribute of the attacker. Another detection method~\cite{sagatov2023countering} is presented that focuses on analyzing outgoing traffic from the victim's server. Through ICMP packet headers, specifically type 3, code 3, in outbound traffic that results from accessing the victim's closed UDP ports, it identifies DNS servers used for amplification attacks.
It is noteworthy that the focus of this study is mitigation strategies and the detection approaches discussed in this section, and the proposed mitigation strategy can be easily incorporated.






\subsection{Mitigation Strategies}
The network's response to the detected threat in order to reduce the impact of the attack can be referred to as a mitigation strategy. Mitigation strategies aim to provide effective countermeasures to minimize downtime and preserve service availability.
WisdomSDN~\cite{abou2020bringing} implements a DNS mitigation scheme that uses rate-limiting techniques for illegitimate DNS traffic and aims to mitigate attacks by dropping DNS requests systematically if the packet rate of illegitimate DNS requests surpasses the threshold. The defense mechanism in the solution proposed by Xing et al.~\cite{xing2016defense} aims to mitigate the attack by dropping packets likewise. 
Sagatov et al.~\cite{sagatov2023countering} propose a mitigation scheme to counter these attacks that employs a temporary traffic-blocking technique from the attack's intermediary server as a mitigation strategy and also suggests another mechanism that involves executing a series of statistical rules for the number of detected packets. However, additional hardware and software components are needed for the SDN protection method. Gupta et al. propose a solution~\cite{gupta2018mitigating} that uses geographically distributed SDN routers and filters incoming traffic, dropping attack packets and allowing only legitimate traffic to reach its destination to minimize the impact of DNS amplification attacks.   
However, the mitigation scheme's reliance on dropping packets carries the inherent risk of also dropping legitimate packets and can potentially impact legitimate users by slowing down or blocking their DNS requests. 
Bohatei~\cite{fayaz2015bohatei} represents an initial research endeavor that employs the usage of SDN and NFV to mitigate DDoS attacks. The primary emphasis of this work is placed on network orchestration to defend against attacks rather than dropping packets. This approach can lead to higher computation overhead due to the additional complexity involved in managing and coordinating multiple components, such as data center and server, in an orchestrated workflow. 
In this study, we implement an approach that employs DNS migration by considering MTD methods as a response to a potential attack mitigation. This approach is not only more flexible for immediate and dynamic adjustment, but it also requires less computation overhead and can avoid the loss of legitimate packets. 

==> methodology0.tex <==
\section{Proposed Approach}
\label{solution}

\subsection{MTD on DNS Flooding Attack}
We implement an MTD approach against DNS flooding attacks. The implementation of MTD on DNS Flooding Attack is provided in this section. The MTD process consists of three parts: matching flows, set actions, and triggering load-balancing. The logic is as follows: 
\begin{enumerate}
    \item First, the system initializes the controller. 
    \item Second, the controller sets a rule to direct DNS traffic to the default DNS server. A response rule is not needed in this case as the default DNS server is the default entry on the host's resolv.conf file.
    \item Third, the controller sets a rule to direct normal flows, including the zone transfer flow, which we will explain later. 
    \item Fourth, the controller periodically fetches the packet count statistics from the set DNS request rule applied to the OVS if the load-balancing status variable is not set to True. We use the OpenFlow Group rule to implement the load-balancing scheme. The Group rule statistics handler needs a different function from the flow rule statistics handler, so that's why we need to have a boolean variable to determine which statistics handler needs to be used. We use the packet count field in the request rule as the indicator of the occurrence of flooding attacks. 
    \item Fifth, the controller calculates the transmission rate of the DNS packets. The transmission rate is calculated by dividing the packet difference by the time window of fetching statistics. The packet difference is calculated by subtracting the previous packet counts from the current packet counts. The value of the transmission rate is used as the threshold for detecting the occurrence of suspicious DNS traffic. 
    \item Sixth, whenever the controller finds the transmission rate of the current flow exceeds the threshold, the controller triggers the DNS load-balancing between the default DNS server and the backup DNS server. This requires the controller to install a response rule that handles the responses generated by the backup DNS server. 
    \item Seventh, if the controller detects the packet rate has dropped from the previous packet rate by 40 percent, it will stop the load-balancing and switch to the default DNS server again.

\end{enumerate} 
The backup DNS server is another DNS server with BIND9 installed and configured as a recursive resolver, and this backup DNS server serves as the secondary DNS server of the default DNS server. This backup DNS server triggers when the pre-set threshold is exceeded. The backup DNS server's job is to help unload a percentage of DNS traffic from the default DNS server. 
Since we implement resiliency instead of dropping packets, load balancing is ideal for resiliency.

Figure \ref{fig:Flow} is the flow chart of the controller.

\begin{figure}[h]
\centering
\includegraphics[width=9cm]{fig/flowchart1.png}
\caption{Controller Flow} 
\vspace{-0.1in}
\label{fig:Flow}
\end{figure}


\subsubsection{DNS Server Management}
We use VBox's command line management tool VBoxManage to manage, automate, and orchestrate the DNS VMs we created. It is a command-line VM management utility. We use this utility to control the startup and stop of the backup server. We have two thresholds. One is for triggering VM startup. Another one is for triggering load balancing. We calculate the VM startup threshold by dividing the load-balancing in half. If the packet rate exceeds the VM startup threshold, the backup server will be started. We will discuss this in detail in the Experimental part.

\subsubsection{Zone File Migration}
We are considering performing a zone file migration to maintain consistency in the DNS zone. The DNS zone file is important. It stores the authoritative name server of a domain. If the backup DNS server does not have the same zone file as the default DNS server, the custom records that are configured in the default DNS server will not be recognized by the backup DNS server. 

% we can talk about amplification attacks in the future work part.....
%\subsection{MTD on DNS Amplification Attack}
%The methodology for detecting DNS amplification attacks is calculating the amplification factor and pairing the response with the corresponding request. The logic behind the pairing scheme is that attackers use spoofed IP addresses and open resolvers to implement the amplification attack. That means the amplified response that targets the victim does not have a corresponding request on the victim's host/resolver.

==> prelim-old.tex <==



\section{Preliminaries}
\label{pre}
In this section, we provide a preliminary information of a few techniques we utilize throughout the rest of the paper and explain the threat model.


%Another one is the DNS amplification attacks. 


%\subsubsection{DNS Amplification}
%DNS amplification attacks are DoS attacks. DNS amplification attacks, as the name suggests, utilize the DNS's vulnerability in that the size of DNS response is larger than the DNS request. DNS amplification attacks also exploit open resolvers as the vehicle to generate large DNS responses. The ratio between the response and the request is called an amplification factor. The larger the amplification factor, the more the difference between the response and the request. To perform a DNS amplification attack, a large amount of specially crafted DNS requests that are intended to generate amplified responses with spoofed IP addresses are sent to one of the open resolvers. The open resolver sends the amplified responses to the target server with the spoofed IP address. The result of the attack is the victim's server is overwhelmed and might cause a service outage.

\subsection{SDN and OpenFlow} 
SDN transforms network management by separating the control logic (control plane) from the underlying hardware responsible for traffic forwarding (data plane). In this configuration, network devices such as switches handle traffic in a direct and simple manner, while a central brain, referred to as the SDN controller, manages the intelligence and decision-making processes. The clear division between control and data planes, along with the concept of flow-based traffic, dramatically simplifies the process of identifying and detecting attacks~\cite{bawany2017ddos}. Moreover, the centralized control allows for quick detection and response. The de facto protocol, OpenFlow~\cite{mckeown2008openflow}, creates the communication infrastructure that allows for direct interaction between the SDN controller and the data plane. This protocol enables the controller to configure packet handling rules in the flow tables of OpenFlow switches. These rules facilitate traffic matching and execution of defined actions, including forwarding, dropping, or modifying traffic. Depending on the rules set by the controller application, an OpenFlow switch can adapt its functionality as a router, switch, firewall, load balancer, and more. 

%Unlike traditional network structures requiring multiple hardware devices to run and manage the network, SDN centralizes the control plane to a controller. It only leaves the data plane, or the virtual switch, for transmitting data. The SDN is constructed by three elements: an SDN controller, an OpenFlow virtual switch (OVS), and hosts connected to the OVS. The job of the control plane is to manage what and how data is being transmitted while the OVS listens to whatever the controller tells it to do. The controller manages the virtual switch by setting OpenFlow (OF) rules. Network admin can add these rules statically using the OpenFlow vSwitch command line tools or by writing scripts to instruct the controller to add rules according to particular situations. We use the latter for our DNS MTD implementation. 

\textbf{Open vSwitch (OVS)}~\cite{pfaff2015design} is a versatile open-source virtual switch that enables bridging and routing between different network environments, which supports OpenFlow and complements SDN architectures. 

The SDN is constructed by three elements: an SDN controller, an OVS, and hosts connected to the OVS. The job of the control plane is to manage what and how data is being transmitted while the OVS listens to whatever the controller tells it to do. The controller manages the virtual switch by setting OpenFlow (OF) rules. Network admin can add these rules statically using the OpenFlow vSwitch command line tools or by writing scripts to instruct the controller to add rules according to particular situations. We use the latter for our DNS MTD implementation. 

\subsection{NFV}
NFV changes the implementation of network components from hardware to software. Instead of running each network component on dedicated hardware, service providers can run all services on a commodity server as Virtual Network Functions (VNFs). The main benefit NFV brings us is scalability. Combined with the programmable OVS, we deploy the DNS servers as VNFs using virtual machines to replicate DNS services~\cite{bari2015orchestrating}. 


\subsection{MTD}
MTD is a technique to constantly change attack surfaces to confuse attackers and impose complexity on performing attacks. MTDs aim to decrease and dynamically adjust the attack surfaces of systems, therefore restricting the possible ways an adversary can exploit to infiltrate a target system~\cite{soule2015quantifying}. It proposes that the target system does not have to stay static but can undergo dynamic changes. This dynamic nature poses a challenge for attackers as they attempt to exploit vulnerabilities while ensuring that the system continues to work for authorized users. MTD utilizes network monitoring tools and system mobility mechanisms to modify the system's configuration in order to prevent the potential damages of  cyberattacks~\cite{carvalho2013mtc2}.

\subsection{Threat Model}
In this paper, DNS flooding is the specific attack vector we focus on mitigating. DNS flooding attacks are DoS attacks that aim to obstruct the availability of the DNS servers, as illustrated in Figure~\ref{fig:attack}. In order to perform a DNS flooding attack, a large volume of DNS requests with randomly generated IP addresses is sent to the target DNS server. The main goal is to exhaust the server's resources, resulting in service disruptions, delays, or complete unavailability. Therefore, the victim machine might be too busy to process those fake DNS requests, so the victim machine can not process legitimate DNS requests. This method is motivated by the intention to deliberately interfere with the regular operation of DNS infrastructure, hence affecting the client's capacity to access online services. The incentive for coordinating botnets~\cite{alieyan2016overview} in DNS flooding operations is the ability to significantly increase the scale of the attack and avoid being detected. Adversaries might strategically utilize compromised devices in a botnet to coordinate and distribute DNS requests on a large scale. This intensifies the effect on specific DNS servers and presents difficulties in identifying and mitigating the attack. 

\begin{figure}[]
%\begin{figure}[h]
\centering
\includegraphics[width=0.8\linewidth]{fig/floodAttack.pdf}
\caption{Threat Model} 
\vspace{-0.1in}
\label{fig:attack}
\end{figure}


%In this paper, we focus on mitigating the DNS flooding attacks. Therefore, DNS Flooding is the specific attack vector in our threat model. DNS flooding attacks are DoS attacks that aim to obstruct the availability of the DNS servers. In order to perform a DNS flooding attack, a large volume of DNS requests with randomly generated IP addresses is sent to the target DNS server. The victim machine might be too busy to process those fake DNS requests such that the victim machine can not process the legitimate DNS requests. The incentive behind DNS flooding attacks lies in the strategic exploitation of vulnerabilities within DNS protocols through distinct attack vectors. During volumetric attacks, adversaries attempt to overwhelm DNS servers by flooding them with a very large number of UDP queries. The main goal is to exhaust the server's resources, resulting in service disruptions, delays, or complete unavailability. This method is motivated by the intention to deliberately interfere with the regular operation of DNS infrastructure, hence affecting the client's capacity to access online services. The incentive for coordinating botnets~\cite{alieyan2016overview} in DNS flooding operations is the ability to greatly increase the scale of the attack and avoid being detected. Adversaries might strategically utilize compromised devices in a botnet to coordinate and distribute DNS requests on a large scale. This intensifies the effect on specific DNS servers and presents difficulties in identifying and mitigating the attack. This attack vector is illustrated in the Figure~\ref{fig:attack}.


==> prelim.tex <==



\section{Preliminaries}
\label{pre}
In this section, we provide a preliminary information of a few techniques we utilize throughout the rest of the paper and explain the threat model.


%Another one is the DNS amplification attacks. 


%\subsubsection{DNS Amplification}
%DNS amplification attacks are DoS attacks. DNS amplification attacks, as the name suggests, utilize the DNS's vulnerability in that the size of DNS response is larger than the DNS request. DNS amplification attacks also exploit open resolvers as the vehicle to generate large DNS responses. The ratio between the response and the request is called an amplification factor. The larger the amplification factor, the more the difference between the response and the request. To perform a DNS amplification attack, a large amount of specially crafted DNS requests that are intended to generate amplified responses with spoofed IP addresses are sent to one of the open resolvers. The open resolver sends the amplified responses to the target server with the spoofed IP address. The result of the attack is the victim's server is overwhelmed and might cause a service outage.

\subsection{SDN and OpenFlow} 
SDN transforms network management by separating the control logic (control plane) from the underlying hardware responsible for traffic forwarding (data plane). In this configuration, network devices such as switches handle traffic in a direct and simple manner, while a central brain, referred to as the SDN controller, manages the intelligence and decision-making processes. 

%The clear division between control and data planes, along with the concept of flow-based traffic, dramatically simplifies the process of identifying and detecting attacks~\cite{bawany2017ddos}. Moreover, the centralized control allows for quick detection and response. The de facto protocol, OpenFlow~\cite{mckeown2008openflow}, creates the communication infrastructure that allows for direct interaction between the SDN controller and the data plane. This protocol enables the controller to configure packet handling rules in the flow tables of OpenFlow switches. These rules facilitate traffic matching and execution of defined actions, including forwarding, dropping, or modifying traffic. Depending on the rules set by the controller application, an OpenFlow switch can adapt its functionality as a router, switch, firewall, load balancer, and more. 

%Unlike traditional network structures requiring multiple hardware devices to run and manage the network, SDN centralizes the control plane to a controller. It only leaves the data plane, or the virtual switch, for transmitting data. The SDN is constructed by three elements: an SDN controller, an OpenFlow virtual switch (OVS), and hosts connected to the OVS. The job of the control plane is to manage what and how data is being transmitted while the OVS listens to whatever the controller tells it to do. The controller manages the virtual switch by setting OpenFlow (OF) rules. Network admin can add these rules statically using the OpenFlow vSwitch command line tools or by writing scripts to instruct the controller to add rules according to particular situations. We use the latter for our DNS MTD implementation. 

\textbf{Open vSwitch (OVS)}~\cite{pfaff2015design} is a versatile open-source virtual switch that enables bridging and routing between different network environments, which supports OpenFlow and complements SDN architectures. 

%The SDN is constructed by three elements: an SDN controller, an OVS, and hosts connected to the OVS. The job of the control plane is to manage what and how data is being transmitted while the OVS listens to whatever the controller tells it to do. The controller manages the virtual switch by setting OpenFlow (OF) rules. Network admin can add these rules statically using the OpenFlow vSwitch command line tools or by writing scripts to instruct the controller to add rules according to particular situations. We use the latter for our DNS MTD implementation. 

\subsection{NFV}
NFV changes the implementation of network components from hardware to software. Instead of running each network component on dedicated hardware, service providers can run all services on a commodity server as Virtual Network Functions (VNFs). The main benefit NFV brings us is scalability. Combined with the programmable OVS, we deploy the DNS servers as VNFs using virtual machines to replicate DNS services~\cite{bari2015orchestrating}. 


\subsection{MTD}
MTD is a technique to constantly change attack surfaces to confuse attackers and impose complexity on performing attacks. MTDs aim to decrease and dynamically adjust the attack surfaces of systems, therefore restricting the possible ways an adversary can exploit to infiltrate a target system~\cite{soule2015quantifying}. %It proposes that the target system does not have to stay static but can undergo dynamic changes. This dynamic nature poses a challenge for attackers as they attempt to exploit vulnerabilities while ensuring that the system continues to work for authorized users. 
MTD utilizes network monitoring tools and system mobility mechanisms to modify the system's configuration in order to prevent the potential damages of cyberattacks~\cite{carvalho2013mtc2}.

\subsection{Threat Model}
DNS flooding attacks are DoS attacks that aim to obstruct the availability of the DNS servers. In order to perform a DNS flooding attack, a large volume of DNS requests with randomly generated IP addresses is sent to the target DNS server. The main goal is to exhaust the server's resources, resulting in service disruptions, delays, or complete unavailability. Therefore, the victim machine might be too busy to process those fake DNS requests, so the victim machine can not process legitimate DNS requests. This method is motivated by the intention to deliberately interfere with the regular operation of DNS infrastructure, hence affecting the client's capacity to access online services. 


%In this paper, we focus on mitigating the DNS flooding attacks. Therefore, DNS Flooding is the specific attack vector in our threat model. DNS flooding attacks are DoS attacks that aim to obstruct the availability of the DNS servers. In order to perform a DNS flooding attack, a large volume of DNS requests with randomly generated IP addresses is sent to the target DNS server. The victim machine might be too busy to process those fake DNS requests such that the victim machine can not process the legitimate DNS requests. The incentive behind DNS flooding attacks lies in the strategic exploitation of vulnerabilities within DNS protocols through distinct attack vectors. During volumetric attacks, adversaries attempt to overwhelm DNS servers by flooding them with a very large number of UDP queries. The main goal is to exhaust the server's resources, resulting in service disruptions, delays, or complete unavailability. This method is motivated by the intention to deliberately interfere with the regular operation of DNS infrastructure, hence affecting the client's capacity to access online services. The incentive for coordinating botnets~\cite{alieyan2016overview} in DNS flooding operations is the ability to greatly increase the scale of the attack and avoid being detected. Adversaries might strategically utilize compromised devices in a botnet to coordinate and distribute DNS requests on a large scale. This intensifies the effect on specific DNS servers and presents difficulties in identifying and mitigating the attack. This attack vector is illustrated in the Figure~\ref{fig:attack}.


==> related-backup.tex <==
\section{Related Work}
Related work is on Sanzida.. Please write up here..

Thank you Sanzida.  -Pei (Thank you! Pei and Professor, for the opportunity to being part of this work.)


Here goes references.


In recent years, the attention of researchers has been captured by SDN-based solutions for combating DDoS attacks in DNS, which aim to detect and mitigate such attacks, predominantly encompassing amplification and flooding attacks. However, the process of detecting and minimizing the attacks poses a significant challenges due to a variety of factors, including the precision of detection, and subsequently, the precision of mitigation.
A solution named WisdomSDN against DNS amplification attack, derived from MTD technique, is proposed in the paper~\cite{abou2020bringing}. This strategy involves mapping between DNS request and response as well as utilizes machine learning algorithm, Bayes classifier, for attack detection based on entropy value which uses network statics collected by sFlow tool. WisdomSDN implements a DNS Mitigation scheme that utilizes meters within OpenFlow switches similar to the proposed strategy to monitor packet speed and uses rate limiting techniques for the illegitimate DNS traffic. This scheme aims to mitigate attacks by discarding DNS requests systematically if the packet speed of illegitimate DNS requests surpasses the threshold. Another machine learning based amplification attack detection scheme is proposed in~\cite{chen2017detecting} that involves an additional hardware to detect the attack increasing overall cost in terms of overhead and equipment. The approach to detect amplification attack in the paper~\cite{aizuddin2017dns} mainly matching query id of DNS request and response to ensure that the DNS response is legitimate using data collected by sFlow and mitigate the attack implementing rate limit in the meter. The threat model of the paper~\cite{ahmed2017mitigating} includes both amplification and flooding attacks and implements Dirichlet process mixture model (DPMM) clustering algorithm to detect attack flows using network statics in OF switches collected by controller periodically.  


Earlier, Xing, et al.~\cite{xing2016defense} present a similar solution as WisdomSDN~\cite{abou2020bringing} that detects DNS amplification attack using packet speed in meter table and entropy calculation. However, this solution uses network statistics in flow table instead of sFlow tool to collect network statics and the utilization of minimal resources is evident as it refrains from employing machine learning. The defense mechanism in this solution aim to mitigate the attack by dropping packet likewise. However, the mitigation scheme's reliance on dropping packets carries the inherent risk of also dropping legitimate packets. Consequently, we implement a approach that employs DNS migration and offers a more viable solution to mitigate attack while preventing the loss of legitimate packets on top of our previous work in~\cite{nesary2022vdns}. 

In the paper~\cite{ozdinccer2019sdn}, a system named YASARA is proposed as a two-phased detection system of DNS Amplification attack that includes a mitigation process but does not focus on it. By monitoring the ratio of the size of the DNS response to that of the corresponding request in first phase and the hop count variation of the client of that DNS in second phase, the system detects attacks. When one these values exceed threshold, the attack is mitigated by dropping all the responses of the corresponding DNS. Bohatei ~\cite{fayaz2015bohatei} represents an initial research endeavor that employs the usage of SDN and NFV to mitigate DDoS attack. Though the attack detection is beyond the scope of this paper and threat model encompasses broader range of DDoS attacks in addition to DNS amplification and flooding, the primary emphasis is placed on network orchestration to defense attack rather than dropping packet. 

Gupta et al. suggests an SDN-based solution ~\cite{gupta2017secure} that detects and neutralizes spoofing involving default DNS Server IP addresses in end hosts, leveraging the flexibility offered by the SDN environment. A DNS DDoS attack prevention mechanism named "KarmaNet" ~\cite{mittal2019karmanet} is proposed which employs SDN's flexibility to reroute DNS response packets enabling self-paralyzing malicious hosts launching DDoS attacks. In a different approach, Gupta et al. proposes a solution ~\cite{gupta2018mitigating} employs a network of geographically dispersed routers called a "Barrier of Routers" (BoR). Using geographically distributed SDN routers, this solution filters incoming traffic, dropping attack packets, and allowing only legitimate traffic to reach its destination to minimize the impact of DNS amplification attacks. They proposed another solution in the paper ~\cite{gupta2019dns} that involves a shareable SDN barrier using a shared bloom filter through OpenFlow switch among all ISP connections of an organisation to detect DNS amplification attack where legitimate DNS requests are added to the bloom filter, and DNS responses passing through the network are checked against it. If a response packet hashes any bit which is set to 0 in the bloom filter, indicates the packet as illegitimate and dropped.  


==> related-bckup2.tex <==
\section{Related Work}
\label{related_work}
In recent years, the attention of researchers has been captured by SDN-based solutions for combating DDoS attacks against DNS, which aim to mitigate such attacks, predominantly encompassing amplification and flooding attacks. The literature on this domain varies, with some studies concentrating on detection, some on mitigation, and a few addressing both. The literature falls within this spectrum and can be categorized into detection strategies and mitigation strategies. The key phases of DDoS mitigation include detection and response phases, and we refer to the solutions that involve response as mitigation strategies in this paper. 
%While detection methods remain relevant, our research primarily contributes to advancing mitigation strategies. However, the process of detecting and minimizing the attacks poses significant challenges due to a variety of factors, including the precision of detection and, subsequently, the precision of mitigation. %The related works of this study can be categorised into detection strategies and mitigation strategies. 

\subsection{Detection Strategies}
Detection strategies entail monitoring patterns in traffic to identify attacks. This is vital to defending DNS against DDoS attacks because the mitigation depends on the output of this phase, and inaccuracies can have an immediate impact on users. A solution named WisdomSDN~\cite{abou2020bringing} is proposed that derived from the MTD technique, involves mapping between DNS request and response as well as utilizes Bayes classifier to identify attack based on entropy analysis. Another machine learning-based amplification attack detection scheme is presented in~\cite{chen2017detecting} that incorporates an additional hardware referred as detecting agent connected to the OpenFlow switch that computes feature vectors of the flows and uses SVM classifier to detect the attack. However, it can increase the overall cost in terms of equipment and overhead. The threat model of the paper~\cite{ahmed2017mitigating} includes both amplification and flooding attacks and implements a Dirichlet process mixture model (DPMM) clustering algorithm to detect attack flows based on network statics in OpenFlow switches collected by the controller periodically. %how they mitigate.  @need more explanation of what they do here..
Xing et al.~\cite{xing2016defense} present a solution that detects DNS amplification attacks using packet rate and entropy calculation. While  minimal resources is evident for this solution as it refrains from employing machine learning, the precision of detection can be lower with constant threshold. A different amplification attack detection approach is proposed by Aizuddin et al.~\cite{aizuddin2017dns} that mainly matches the DNS request ID with the response to ensure that the DNS response is legitimate. %and mitigate the attack implementing rate limit in the meter. 
Kim et al.~\cite{kim2017preventing} describe a DNS amplification attack mitigation system that can identify orphan DNS responses using a one-to-one strict mapping scheme between DNS requests and responses at OpenFlow switch and controller and drop these responses to mitigate attack. Gupta et al.~\cite{gupta2019dns} propose a solution that involves a shareable SDN barrier using a shared bloom filter through OpenFlow switch among all ISP connections of an organisation to detect DNS amplification attack where legitimate DNS requests are added to the bloom filter, and DNS responses passing through the network are checked against it. If a response packet hashes any bit which is set to 0 in the bloom filter, indicates the packet as illegitimate and dropped. A two-phased detection method for DNS amplification attacks called YASARA~\cite{ozdinccer2019sdn} is proposed that detects attack by monitoring the ratio of DNS response size to the corresponding request and DNS client's hop count variation. When one of these values exceeds the threshold, the attack is mitigated by dropping all the responses of the corresponding DNS. On the other hand, Lyu et al.~\cite{lyu2021hierarchical} address the issue of DNS attacks on enterprise networks, utilizing trained and anomaly-based detection models to identify flooding attacks and scans from external sources of attacks instead of victims. They introduce a  hierarchical and dynamic graph data structure for scalable monitoring to find the key attribute of attacker. Another detection method~\cite{sagatov2023countering} is presented that focuses on analyzing outgoing traffic from the victim's server. Through ICMP packet headers, specifically type 3, code 3, in outbound traffic that results from accessing the victim's closed UDP ports, it identifies DNS servers used for amplification attacks.
It is noteworthy that, the focus of this study is mitigation strategies and the detection approaches discussed in this section and the proposed mitigation strategy can be easily incorporated.

\subsection{Mitigation Strategies}
The network's response to the detected threat in order to reduce the impact of the attack can be referred to as a mitigation strategy. Mitigation strategies aims to provide effective countermeasures to minimize downtime and preserve service availability.
WisdomSDN~\cite{abou2020bringing} implements a DNS mitigation scheme that uses rate-limiting techniques for illegitimate DNS traffic and aims to mitigate attacks by dropping DNS requests systematically if the packet rate of illegitimate DNS requests surpasses the threshold. The defense mechanism in the solution proposed by Xing et al.~\cite{xing2016defense} aims to mitigate the attack by dropping packets likewise. 
Sagatov et al.~\cite{sagatov2023countering} propose a mitigation scheme to counter these attacks that employs a temporary traffic-blocking technique from the attack's intermediary server as a mitigation strategy and also suggested another mechanism that involves executing a series of statistical rules for the number of detected packets. However, additional hardware and software components are needed for the SDN protection method. Gupta et al. proposes a solution~\cite{gupta2018mitigating} that use geographically distributed SDN routers and filters incoming traffic, dropping attack packets, and allowing only legitimate traffic to reach its destination to minimize the impact of DNS amplification attacks.   
However, the mitigation scheme's reliance on dropping packets carries the inherent risk of also dropping legitimate packets and can potentially impact legitimate users by slowing down or blocking their DNS requests. 
%The SDN-based mitigation techniques for DDoS attacks in DNS mainly includes dropping suspicious network traffic and rate limiting for incoming requests to reduce the impact of DDoS attack in DNS. Both of this approach can potentially impact legitimate users by slowing down or blocking their DNS requests. 
Bohatei~\cite{fayaz2015bohatei} represents an initial research endeavor that employs the usage of SDN and NFV to mitigate DDoS attacks. The primary emphasis of this work is placed on network orchestration to defend against attacks rather than dropping packets. These approach can lead to higher computation overhead due to the additional complexity involved in managing and coordinating multiple components such as data center and server in an orchestrated workflow. 
In this study, we implement an approach that employs DNS migration by redirecting traffic as a response to attack detection on top of our previous work in~\cite{nesary2022vdns}. This approach is not only more flexible for immediate and dynamic adjustment, but it also requires less computation overhead and can avoid the loss of legitimate packets. 
% A DNS DDoS attack prevention mechanism named KarmaNet~\cite{mittal2019karmanet} is proposed which employs SDN's flexibility to reroute DNS response packets enabling self-paralyzing malicious hosts launching DDoS attacks. Paper quality? 

 %@what is difference from our work?




%DNS spoofing
%Each DNS request is given an authentication packet after being stalled for a short while, as part of a collaborative authentication (CAuth)~\cite{sahri2016collaborative} method, DNS requests are accepted provided the client answers to the authentication packet. 
